LSST Science Book, Version 2.0

A survey that can cover the sky in optical bands over wide fields to faint magnitudes with a fast cadence will enable many of the exciting science opportunities of the next decade. The Large Synoptic Survey Telescope (LSST) will have an effective aperture of 6.7 meters and an imaging camera with field of view of 9.6 deg^2, and will be devoted to a ten-year imaging survey over 20,000 deg^2 south of +15 deg. Each pointing will be imaged 2000 times with fifteen second exposures in six broad bands from 0.35 to 1.1 microns, to a total point-source depth of r~27.5. The LSST Science Book describes the basic parameters of the LSST hardware, software, and observing plans. The book discusses educational and outreach opportunities, then goes on to describe a broad range of science that LSST will revolutionize: mapping the inner and outer Solar System, stellar populations in the Milky Way and nearby galaxies, the structure of the Milky Way disk and halo and other objects in the Local Volume, transient and variable objects both at low and high redshift, and the properties of normal and active galaxies at low and high redshift. It then turns to far-field cosmological topics, exploring properties of supernovae to z~1, strong and weak lensing, the large-scale distribution of galaxies and baryon oscillations, and how these different probes may be combined to constrain cosmological models and the physics of dark energy.

==> Makefile <==
all: pdf

# Really clean should clean here and in subdirectories
# Most notably it should at least clean .blg and .bbl files
cleanall:
	-rm -f  *.aux *.log *.dvi *.blg *.bbl *.inx *.aut *.toc *.out SciBook.pdf
	-rm -f  */*.aux */*.log */*.dvi */*.blg */*.bbl */*.inx */*.aut */*.toc */*.out 
	-rm -f  */*/*.aux */*/*.log */*/*.dvi */*/*.blg */*/*.bbl */*/*.inx */*/*.aut */*/*.toc */*/*.out 

#clean everything except the pdf file.
cleanup:

# No longer needed if SciBook.pdf is removed anyway...
# trash: clean
# 	-rm -f SciBook.pdf
# 
# force: trash SciBook.pdf

pdf: SciBook.pdf

ps: SciBook.pdf
	pdf2ps SciBook.pdf

TEXFILES = *.tex */*.tex */*/*.tex
#BIBFILES = general.bib */*.bib
BIBFILES = */*.bib

check:
	./checkbook.csh

# Problem: how to get current version number?

# Old code, based on svn status call:
# # This pulls out the version number and stamps it on the front cover.
# # You have to type your password (twice) so only do it when making final!
# versiondate:
# 	(echo '\begin{center}') > VersionDate.tex
# 	(svn status --show-updates --verbose wc | sed 's/Status against revision: /Version /') >> VersionDate.tex
# 	(echo ' ') >> VersionDate.tex
# 	(date +"%B %d, %Y") >> VersionDate.tex
# 	(echo '\end{center}') >> VersionDate.tex
# 
# # Have to have something in VersionDate.tex! Here's a dummy version, date but
# # no version number:	
# dummyversiondate:
# 	(echo '\begin{center}') > VersionDate.tex
# 	(echo 'Draft Version') >> VersionDate.tex
# 	(echo ' ') >> VersionDate.tex
# 	(date +"%B %d, %Y") >> VersionDate.tex
# 	(echo '\end{center}') >> VersionDate.tex

# New code (PJM 2009-01-29), based on contents of entries file.
# Differences between mac and linux in how echo deals with escape chars,
#   switched to clunkier cat commands (PJM 2009-02-09)
# 2009/05/24 - MWV: The '-n' from the echo was ending up in the 'VersionDate.tex' file
#                   Under Bash 'echo' is /bin/echo.  Under Tcsh 'echo' is a shell command.
#                   Changing things to always use /bin/echo worked.  
#                   This seems a safe-enough assumption but I don't like having to make it.
versiondate:
	(cat VersionDate.begin) > VersionDate.tex
	(/bin/echo -n "Version "; tail -n +4 .svn/entries | head -1 | sed -e 's/-n//') >> VersionDate.tex
	(echo ' ') >> VersionDate.tex
	(date +"%B %d, %Y") >> VersionDate.tex
	(cat VersionDate.end) >> VersionDate.tex
 
# Note: VersionDate.tex MUST exist for SciBook to compile! 
SciBook.pdf: cleanall versiondate SciBook.tex SciBook.sty $(BIBFILES) $(TEXFILES)
	pdflatex SciBook.tex
	bibtex common/common
	bibtex agn/agn
	bibtex common/common
	bibtex cosmological_physics/Cosmological_physics
	bibtex design/design
	bibtex epo/epo
	bibtex galaxies/galaxies
	bibtex introduction/introduction
	bibtex lss/lss
	bibtex milkyway/milkyway
#	bibtex performance/performance
	bibtex solarsystem/solarsystem
	bibtex stellarpops/stellarpops
	bibtex stronglens/stronglens
	bibtex supernovae/supernovae
	bibtex transients/transients
	bibtex weaklens/weaklens
	bibtex appendix/assumed_cosmology
	bibtex appendix/analysis/analysis
	bibtex appendix/acronym/acronyms
	pdflatex SciBook.tex
	pdflatex SciBook.tex
	pdflatex SciBook.tex
	rm -f  *.aux *.log *.dvi *.inx *.aut *.out
	rm -f  */*.aux */*.log */*.dvi */*.inx */*.aut */*.out 
	rm -f  */*/*.aux */*/*.log */*/*.dvi */*/*.inx */*/*.aut  */*/*.out 

# Generate finalised version of the book, with no line numbers:
final: setfinal SciBook.pdf

# Generate draft version of the book, with line numbers, 
# and restore default (final) settings afterwards:
draft: setdraft SciBook.pdf setfinal

# Fiddling needed by previous options:
setfinal:
	cat SciBook.sty | sed s/'setboolean{draft}{true}'/'setboolean{draft}{false}'/g > junk
	mv junk SciBook.sty
	echo "*** SciBook.sty edited for final version ***" >& /dev/null

setdraft:
	cat SciBook.sty | sed s/'setboolean{draft}{false}'/'setboolean{draft}{true}'/g > junk
	mv junk SciBook.sty
	echo "*** SciBook.sty edited for draft version ***" >& /dev/null



==> VersionDate.tex <==
\begin{center}
Version  
November 30, 2009
\end{center}


==> design/Data_Management_and_Products.tex <==
\section{Data Management and Products}

{\it (Tim Axelrod, Jeff Kantor, Gregory Dubois-Felsmann)}

The unique but enabling challenge for the LSST Observatory is to provide fully 
calibrated public databases to the user community in a way that facilitates the 
frontier science described in Chapter \autoref{chp:design} but without precluding new lines of 
research that cannot be anticipated today. The nature, quality, and volume of 
LSST data will be unprecedented. Each patch of sky will be visited 1000 times 
(2$\times$15 sec exposures) in ten years. With 20 trillion photometric and temporal 
measurements covering 20 billion detected objects, this will produce the world's 
largest non-proprietary database. New algorithms will have to be developed and 
existing approaches refined in order to take full advantage of this resource. In 
this section, we describe the reference design for the LSST data management 
system (DMS).
The LSST data management system will be a world-class computational facility 
that will process and deliver LSST data to meet these challenges. The computational 
facilities and data archives of the LSST DMS will rapidly make it one of the largest 
and most important facilities of its kind in the world. To tackle these challenges 
and to minimize risk, LSSTC and the data management subsystem team have taken 
four specific steps:

\begin{itemize}
  \item The National Center for Supercomputing Applications (NCSA) at the 
    University of Illinois at Champaign-Urbana will serve as the primary LSST archive 
    center; the Infrared Processing and Analysis Center (IPAC) at the California 
    Institute of Technology will develop custom software and review software baseline 
    costing models; 
    Lawrence Livermore National Laboratory (LLNL) and Stanford Linear Accelerator Center (SLAC) 
    led the effort to size and design the computational infrastructure and database system. 
    Google Corporation is providing advice and collaborating on file system structures and public data access.

  \item The DM team has closely examined and continues to monitor relevant developments within, 
    and recruited key members from, precursor astronomical surveys including 
    2MASS, SDSS, the ESSENCE and SuperMACHO projects, the Deep Lens Survey, and the NVO.

  \item The DM team is monitoring relevant developments within the physics community 
    and has recruited members with experience in comparable high energy physics data 
    management systems. Specifically, members were recruited from the BaBar 
    collaboration at SLAC and the Atlas collaboration at BNL.

  \item The DM team defined four basic ``Data Challenges'' (DC) to evaluate and certify 
    the LSST DM architecture. Success with these challenges prior to the beginning of 
    construction will provide confidence that DM budget, schedule, and technical 
    performance targets will be acheved.

\end{itemize}

\subsection{The technical challenges in DM}

\subsection{ Data Access and Computing Requirements (query and computing)}

\subsection{Data products and release (catalogs and images)}

\subsection{DM Architecture}

\subsection{Requirements and Deliverables of the Data Management System}

The LSST Data Management System (DMS) will deliver:
\begin{itemize}
  \item {\bf Image archives:} An image data archive of over two million 
    raw and calibrated 12 GB scientific images, each image available within 24 hours of capture.
  \item {\bf Alerts:} Verified alerts of transient and moving objects detected within 
    60 seconds of the image capture (30 s goal)
  \item {\bf Catalogs:} Astronomical catalogs containing billions of stars and galaxies, 
    richly attributed in both time and space dimensions and setting a new standard in 
    uniformity of astrometric and photometric precision. This includes a query toolkit 
    with associated computational, storage, and communications infrastructure.
  \item {\bf Quality Assurance:} A process including documentation to ensure 
    data integrity with full tracking of data provenance.
\end{itemize}


\subsection{Computational Sizing}

In order to balance between near-real time and non-real time requirements, we have divided 
computing across four specialized facilities: 
Mountain Summit, Base Facility, Archive Center, and Data Access Centers. 
The total processing requirements for LSST start at approximately 100 TFLOPS in the 
commissioning period and first survey year and then grow linearly. 
These requirements are technically feasible now. 
The growth trend is less steep than industry trends in computing system throughput.
Though LSST processing requirements are considerable by the standards of 
current optical/infrared astronomical surveys, they are fairly modest 
when compared to the requirements of high energy physics, radio astronomy, 
and other scientific programs driving the top 500 supercomputing sites).

The sizing of the computational requirements involves a conscious trade-off 
between the cost of saving all computed data products at all stages of processing 
vs. re-computing data products on demand. This resulted in a CPU-intensive model 
because image data expands from 15TB to over 100TB per night upon processing. 
Transferring/storing 100TB per night is cost-prohibitive; computing system 
throughput trends support the required re-processing cost effectively.

The strategy adopted requires that data be reduced at the Base Facility in 
order to meet alert latency requirements; raw image data and metadata are 
transferred to the Archive Center, where they are processed again. 
Only certain data products and the provenance needed to re-create the other 
data products on demand are stored permanently. Before every data release, 
all data previously processed are re-processed with the latest algorithms, 
calibration products, and parameters. Finally, the system is sized to support 
on-the-fly, ``smart'' re-processing of as yet unreleased data for other needs, 
such as end-user science. 
This includes regenerating individual reduced frames when necessary.

\subsection{Input/Output Sizing}

LSST data storage requirements are substantial:
LSST will reach multi-petabyte scale during the first year of operations. 
While the image data will grow at a steady 6 petabytes/year based on 
observing cadence and image size, a significant portion of the catalog 
data growth is a direct result of observing near or in the Galactic plane. 
The largest of the catalogs, the Source Catalog, will hold about 250 billion 
source measurements in the first data release (DR1) and 6.5 trillion in the 
last data release (DR10). Image data will be released on a daily
basis and catalog data will be released twice in the first year and once 
each year thereafter, with DR1 projected for release in 2014. 
Once released, all data products will be permanently stored and immutable. 
Unreleased data collected and processed between releases will be updated 
nightly and will be immediately available; these data will carry the {\it caveat} 
that analytical results based on that data may be non-reproducible once the 
data are re-processed for inclusion in the new DR.



==> design/OpSim.tex <==
% ======================================================================
%+
% NAME:
%   OpSim.tex
%
% PURPOSE:
%   Operations Simulator section for SciBook
%
% COMMENTS:
%    
% INPUTS:
%
% OPTIONAL INPUTS:
%
% OUTPUTS:
%
% DEPENDENCIES:
%
% EXAMPLES:
%   
% BUGS:
%
% AUTHORS:
%  Taken from the 2008 Overview Paper, Ivezic et al.
% ======================================================================

\section{Operations Simulator}
\label{sec:design:opsim}

{\it Philip Pinto, \v Zeljko Ivezi\'c, Abhijit Saha, Kem Cook, R. Lynne Jones}

The LSST Operations Simulator creates realizations of the set of
observations (visits) that the LSST will make over its 10-year
lifetime.  It contains detailed
models of site conditions and hardware and software performance, and
an algorithm for scheduling observations which will, eventually, drive
the largely robotic observatory.  Its output includes a detailed list
of visits for a realization of the entire survey lifetime, including
estimates of the depth of the stacked image in a given filter as a
function of position (\autoref{fig:design:rband}). 

Observing conditions include a model for seeing
drawn from the data shown in \autoref{fig:design:seeing}. This model
includes
% from an extensive body of on-site MASS/DIMM
%(Multi-Aperture Scintillation Sensor and Differential Image
%Motion Monitor) measurements obtained during site
%selection and characterization. It not only
%reproduces the observed seeing distribution, but includes
the auto-correlation spectrum of seeing with time over intervals
from minutes to seasons. Weather data (including its correlations) are taken
from ten years of hourly measurements at nearby Cerro
Tololo. 
%The time history of site conditions is important
%if the simulation is to faithfully reproduce a sequence
%of observations. Thus, for example, 
Thus the simulator correctly
represents the variation of limiting magnitude between
pairs of observations used to detect NEOs and the
correlation between, for example, seasonal weather patterns
and observing conditions at any given point on the
sky. The signal-to-noise ratio of each observation is determined
using a sky background model, which includes
the dark sky brightness in each filter, the effects of seeing
and atmospheric transparency, and a detailed model for
scattered light from the moon and/or twilight at each
observation. The time taken to move from one observation
to the next is given by a detailed model of the
camera, telescope, and dome. It includes such effects as
the acceleration/deceleration profiles employed in moving
in altitude, azimuth, camera rotator, dome azimuth,
and wind/stray light screen altitude, the time taken to
damp vibrations excited by each slew, cable wrap, time
taken for active optics lock and correction as a function
of slew distance, filter change, and focal plane readout.

Observations are scheduled by a ranking algorithm.
After a given exposure, all possible next observations
are assigned a score, which depends upon their locations,
times, and filters according to a set of scientific requirements
that can vary with time and location. For example,
if an ecliptic field has been observed in the $r$ band,
the score for another $r$-band observation of the same field
will initially be quite low, but it will rise in time to peak
about an hour after the first observation, and decline
thereafter. This results in these observations being acquired
as pairs roughly an hour apart, which enables efficient 
association of NEO detections. To ensure uniform
sky coverage, fields with fewer previous observations will
be scored more highly than those that have already
been observed more frequently.

Once all possible next observations have been scored
for scientific priority, their scores are modified according
to observing conditions (e.g., seeing, airmass, and sky
brightness) and to criteria such as low slew time to move
from the current position, time spent to change filters,
etc. The highest ranked observation is then performed,
and the cycle repeats. The result of a simulator run
is a detailed history of which locations on the sky were
observed when, in what filter, and with what sky background,
seeing and other observing conditions. It takes
about a week to produce a decade-long simulation using
an average PC.



==> design/calibration_v3.tex <==
\section{Photometric Calibration}
\label{sec:design:calsim}

{\it David Burke, Tim Axelrod, James G. Bartlett, David Cinabro, Chuck
Claver, James Frank, John Haggerty, \v Zeljko Ivezi\'c, R. Lynne Jones,
Brian Meadows, David Monet, Bogdan Popescu, Abhijit Saha, Michael
Sivertz, J. Allyn Smith, Christopher Stubbs, Tony Tyson}


The LSST specifications for the precision of photometric calibration
are a factor of two more stringent than typically achieved in previous
surveys, and have been approached only in limited photometric
conditions, for example, by the Sloan Digital Sky Survey (SDSS,
\citealt{Ive++07}).  They are especially demanding given the LSST's
very wide field of view, its relatively short exposures, and the fact
that the LSST exposes in typically only two filters per night across
most of the sky.  And these specifications must be met for all
conditions in which LSST is observing, not just on ``photometric''
nights.

\iffalse
Ideally the LSST Object Catalog would contain broadband magnitudes of
celestial objects derived from the integral of the source specific
flux {\it at the top} of the earth's atmosphere, $F_\nu(\lambda)$
(Jy), weighted by a fixed well-defined standard optical bandpass
$\phi_b^{std}(\lambda)$,
\begin{equation}
\label{eqn:Fstd}
  F_b^{std} = \int_0^\infty {F_\nu(\lambda) \phi_b^{std}(\lambda) d\lambda}.
\end{equation}
The dimensionless normalized response function is defined as 
\begin{equation}
\label{eq:design:PhiStd}
    \phi_b^{std}(\lambda) \equiv {\frac{T_b^{std}(\lambda) \lambda^{-1}}{ \int_0^\infty {T_b^{std}(\lambda) \lambda^{-1} d\lambda}}}
\end{equation}
where $T_b^{std}(\lambda)$ is a standard system response (correspoding
to combined effects of the earth's atmosphere and the LSST system). 
The weight $\lambda^{-1}$ reflects the fact that the CCDs used as
sensors in the camera are photon-counting devices rather than
calorimeters.  The units for $F_b^{std}$ are Jansky, and by
definition, $\int_0^\infty {\phi_b^{std}(\lambda) d\lambda}=1$.  
A corresponding astronomical magnitude is defined as
\begin{equation}
\label{eqn:stdmag}
   m_b^{std} \equiv -2.5\log_{10}\left({\frac{F_b^{std}}{F_{AB}}}\right)
\end{equation}
The flux normalization $F_{AB} = 3631$ Jy (1 Jansky = 10$^{-26}$ W
Hz$^{-1}$ m$^{-2}$ = 10$^{-23}$ erg cm$^{-2}$ s$^{-1}$ Hz$^{-1}$)
follows the standard of \citet{Oke+Gunn83}.
\fi 

A ground-based telescope and photometric camera system can only measure
the integral of the optical flux density $F_\nu$ from a celestial object {\it at the top of the atmosphere} 
weighted by an observational bandpass, $T_b(x,y,alt,az,t,\lambda)$,
\begin{equation}
\label{eqn:Fo}
             C_b^{meas} = A \Delta T \int_0^\infty {F_\nu(\lambda) T_b(x,y,alt,az,t,\lambda) \lambda^{-1} d\lambda},
\end{equation}
where the $C_b^{meas}$ are digitized counts (ADU) recorded on an image in exposure time $\Delta T$
through a telescope with aperture $A$.
The observational bandpass is the combined transmittance of the atmosphere and the instrumental
throughput of the telescope and camera (including the optical filter $b$).
In general it is a complicated function of the coordinates $(x,y)$ of the
source image in the focal plane of the camera, the altitude and azimuth $(alt,az)$ of the pointing of the telescope,
and the time (and date) $t$ of the observation.
\iffalse
\begin{equation}
\label{eqn:SDef}
         T_b(x,y,alt,az,t,\lambda) = T_b^{sys}(x,y,t,\lambda) \times T_b^{atm}(alt,az,t,\lambda), 
\end{equation}
where $T_b^{atm}$ is the optical transmittance from the top of the
atmosphere to the input pupil of the telescope, and $T_b^{sys}$ is the
instrumental system response (``throughput'') from photons through the
input pupil to detector.
\fi
Removal of spatial and temporal variations in the measured
counts that arise from changes in the observational bandpass, and ultimate calibration of ADU counts to
a physical scale, are challenges for the observational astronomer.

Traditionally, a measure of
the bandpass of a particular observation is obtained by interleaving science
targets with observations of standard stars over a range of airmass
throughout the observing night.
This provides the convolution of $T_b$ with the SEDs of the standard stars, and combined
with an appropriate flat-field for the instrument, it can be used to make an approximation of
the observational bandpass at the coordinates of the science observations.
%This approximation can then be used for interpretation
%of the measurements made of the science targets.  A night is generally
%regarded as ``photometric'' if multiple observations of targets yield
%sufficiently small variations in measured magnitudes.  It is found
%that some nights are 1\% nights, and some nights are 2\% nights, but
%it is only very rarely better.  The specifications for LSST photometry
%given in the Science Requirements Document (SRD, \citet{Ive++07}) are
%more strict than this will allow.  Furthermore, goals for the
%efficiency of the LSST survey require that SRD specifications be met
%in observing conditions that would not traditionally be called
%``photometric''.  So LSST will take a non-traditional approach to
%photometric measurement \citep{S+T06}.
Given the stringent requirements for photometric calibration
(\autoref{sec:introduction:reqs}), however, this approach will not be adequate for LSST,
and we approach this calibration problem anew.  
 
The LSST facility will include auxiliary subsystems to independently
measure atmospheric transmittance and the instrumental response with
good precision and fine temporal, spectral, and spatial resolution.
The system response (i.e., the fraction of photons hitting the primary
mirror that are recorded, as a function of wavelength) will be
measured {\it in situ} using a dome projector system that is
illuminated with a tunable monochromatic light source.
\iffalse
  The relative
dependence of the flux of light from this screen as a function of
wavelength will be monitored with a photodiode calibrated externally
to allow the shapes of the LSST instrumental bandpasses to be
precisely measured \citep{S+T06}.
\fi
The atmospheric transmittance will be measured 
using spectroscopic observations of bright isolated stars made with an
auxiliary telescope placed near the LSST on Cerro Pach\'on (\autoref{fig:design:telescope_artist}).
\iffalse
This telescope will repeatedly observe a small set of stars as they
traverse the sky during the nights they are visible.  The variations
of the observed spectra with airmass will be combined with a
state-of-the-art physical atmospheric model and readily available
computer codes to extract the atmospheric absorption present during LSST
operations \citep{Bur08}.
\fi
These systems are designed to provide
well-defined and precise measurements for each LSST observation; they are discussed further below. 

With the information that will be provided by the LSST auxiliary instrumentation,
a {\it measured} bandpass for each observation made with the main telescope will be computed,
\begin{equation}
\label{eqn:SmeasDef}
      S_b^{meas}(x,y,alt,az,t,\lambda) = S_b^{sys}(x,y,t,\lambda) \times S^{atm}(alt,az,t,\lambda),
\end{equation}
where $S_b^{sys}$ (ADU/photon) is the {\it measured} instrumental
system response, and $S_b^{atm}$ (dimensionless) is the {\it measured} atmospheric transmittance.  
From these measurements a {\it measured} top-of-the-atmosphere in-band source flux can be
defined,
\begin{equation}
\label{eqn:ABmag}
  F_b^{meas} \equiv \frac{C_b^{meas}}{A \Delta T \int_0^\infty {\lambda^{-1} S_b^{meas}(\lambda) d\lambda }},
\end{equation}
and a corresponding astronomical magnitude will be defined by normalizing the measured flux to a source with a flat SED,
\begin{equation}
\label{eqn:stdmag}
   m_b^{meas} \equiv -2.5\log_{10}\left({\frac{F_b^{meas}}{F_{AB}}}\right).
\end{equation}
The flux normalization $F_{AB} = 3631$ Jy (1 Jansky = 10$^{-23}$ erg cm$^{-2}$ s$^{-1}$ Hz$^{-1}$)
follows the standard of \citet{Oke+Gunn83}.
\iffalse
It is convenient to also define a {\it measured} normalized response function,
\begin{equation}
\label{eq:design:PhiDef}
    \phi_b^{meas}(\lambda) \equiv {\frac{S_b^{meas}(\lambda)
    \lambda^{-1}}{\int_0^\infty {S_b^{meas}(\lambda)
    \lambda^{-1} d\lambda}}}. 
\end{equation}
\fi
In full, the LSST photometry will be described by individual measurements of $S_b^{meas}$ and the
corresponding $m_b^{meas}$.  The survey will collect $\sim$10$^{12}$
such ($S_b^{meas}$,$m_b^{meas}$) pairs over a ten year period --
one pair for each source detected in each image.

\subsection{  Measurement of Instrumental System Response $S_b^{sys}$  }
\label{sec:sys}

A monochromatic dome projector system will be used to provide a well-controlled source of light for 
measurement of the relative throughput of the full LSST instrumental system.
This includes the reflectivity of the mirrors, transmission of the refractive optics and filters,
the quantum efficiency of the sensors in the camera, and the gain and linearity of the sensor read-out electronics.

An array of projectors mounted in the dome of the LSST enclosure will be illuminated with both broadband
(e.g. quartz lamp) and tunable monochromatic light sources.
These ``flat-field'' projectors are designed to fill the LSST \'etendue with uniform illumination,
and also to limit the extent of stray light emitted outside the design acceptance of the system.
A set of precision diodes will be used to normalize the photon flux integrated during flat-field exposures.
These photodiodes, together with their read-out electronics, will be calibrated at the U.S. National Institute of Standards (NIST)
to $\sim 0.1\%$ relative accuracy across wavelength from 450 nm to 950 nm.
The response of these diodes varies smoothly across this range of wavelength and provides a well-behaved reference \citep{stubbs05}.
Adjustment of the wavelength of the light source can be as fine as one nanometer, and will
allow precise monitoring of the shape of the bandpasses of the instrumental system during the course of the survey \citep{S+T06}.

It is anticipated that the shapes of the bandpasses will vary only slowly, so detailed measurement will need be done only once per month or so.
But build-up of dust on the surfaces of the optics will occur more rapidly.  
The dimensions of these particles are generally large, and their shadows will be out of focus at the focal plane.
So the loss of throughput due to them will be independent of wavelength - i.e. ``gray'', and the pixel-to-pixel gradients of their shadows will not be large. 
Daily broadband and ``spot-checks'' at selected wavelengths with the monochromatic source will be used to measure day-to-day changes in the system passbands.  

\subsection{  Measurement of Atmospheric Transmittance $S^{atm}$  }
\label{sec:atmo}

\iffalse
Precise photometry is traditionally done only during times when atmospheric conditions are stable and clear of clouds.
Only a fraction of the observing time is ``photometric'', and even identification of such conditions can be ambiguous.
The LSST survey must maximally utilize all available time.
Dedicated hardware systems and supporting software will be used to rigorously and precisely measure atmospheric opacity and to extend periods of 
successfull LSST operations to include conditions that would not be traditionally ``photometric''.
It is likely that SRD design goals can be met even when observing through up to a full magnitude of atmospheric extinction.
\fi

Many studies have shown that atmospheric transmission can be factored into the product of
a frequency dependent (``non-gray'') part that varies only on spatial
scales larger than the telescope field-of-view and temporal scales long compared with the interval between LSST exposures;
and a frequency independent part (``gray'' cloud cover) that varies on moderately short spatial scales (larger than
the PSF) and temporal scales that may be shorter than the interval between exposures:
\begin{equation}
\label{Eq:satmo}
S^{atm}(x,y,alt,az,t,\lambda)~=~T_{g}(x,y,alt,az,t) \times T_{ng}(alt,az,t,\lambda).
\end{equation}

\noindent The measurement strategies to determine $T_g$ and $T_{ng}$ are quite different:
\begin{itemize}
\item $T_{ng}$ is determined from repeated spectroscopic measurements of a small set of probe stars by a dedicated auxiliary telescope.
\item $T_{g}$ is determined from the LSST science images themselves, first approximately as each image is processed, and later more
precisely as part of a global photometric self-calibration of the survey.
The precise measurement of $T_{g}$ is based on the measured fluxes of
a very large set of reference stars that cover the survey area and are
observed over many epochs.  
Every exposure contains a large enough set of sufficiently stable
stars that a spatial map can be made of $T_{g}$ across each image.
\end{itemize}

The LSST design includes a 1.2m auxiliary calibration telescope
located on Cerro Pach\'on near the LSST that will  
be used to measure $T_{ng}(alt,az,t,\lambda)$.
The strategy is to measure the full spatial and temporal variation in atmospheric extinction throughout each night
independently of operations of the main survey telescope. %  \cite{lsstdoc5367}.
This will be done by repeatedly taking spectra of a small set of probe stars as they traverse the sky each night.
These stars are spaced across the sky to fully cover the area surveyed by the LSST main telescope.
The calibration will use state-of-the-art atmospheric models
\citep{Stubbs++07} and readily-available codes (MODTRAN4) to
accurately compute  
the signatures of all significant atmospheric components in these spectra.
This will allow the atmospheric mix present along any line of sight at any time to be interpolated from the measured data.
The probe stars will be observed many times during the LSST survey, so the SED of each star can be bootstrapped from the data.
The instrumental response of the spectrograph can also be bootstrapped
from the data by including stars with a variety of SEDs over a broad
range of airmass. 

\iffalse
Recognition of the signatures of atmospheric components can be done with relatively modest spectral resolution (R $\sim$ 400),
but it is important that the full spectral range (330nm to 1100nm) be obtained in a single exposure.  
To keep up with changes in the atmospheric mix (particularly water vapor), this subsystem must be able to slew and capture spectra
of relatively bright stars ($r<12$) at a reasonable pace (every 5 minutes).
An iterative fitting procedure is used to extract parameters (effective temperature, gravities, and luminosities) for
each of the probe stars (once per Data Release), nightly corrections for the spectrograph efficiency, and coefficients
that define the mix of constituents in the atmosphere.
The Auxiliary Telescope is designed to take spectra fast enough that the atmospheric extinction for each LSST pointing can
be interpolated from the data from the probe stars.
\fi

\subsection{Calibration Procedure}
\label{Sec:calproc}

Two levels of LSST calibration will be carried out at differing
cadences and with differing performance targets.  A nightly data
calibration based on the best available set of prior calibrated
observations will provide ``best-effort'' precision and accuracy.
This calibration will be used for quality assurance, generation of
alerts to transients, and other
quantities appropriate for Level 1 Data Products
(\autoref{sec:design:dataproduct}). 
A more complete analysis will
recalibrate the data accumulated by the survey at periodic ``Data
Release'' dates (Level 2 in the terminology of
\autoref{sec:design:dataproduct}).  It is this repeated calibration of
the accumulated 
survey that will be held to the survey requirements for photometric
repeatability, uniformity, and accuracy.  
%This section describes the
%measured calibration data and their use in the Data Release
%calibration process (\autoref{Fig:DRmeasures}).

\iffalse
[MORE DETAIL THAN WE NEED.]
\begin{figure}[hbt]
\begin{center}
\includegraphics[width=1.0\hsize,clip=true]{design/figs/LSST_DR_Measured_Data.png}
\caption{Measured data products used in the LSST Data Release calibration process.
The quantities are defined in the text.}
\label{Fig:DRmeasures}
\end{center}
\end{figure}
\fi

A set of LSST ``standard'' bandpasses $\phi_b^{std}(\lambda)$ will be defined
as the suitably weighted mean of the measured bandpasses encountered during the commissioning
(and perhaps first observing runs) of the LSST observatory.
%%An example of a plausible standard bandpass is shown in
%%\autoref{Fig:phiChange}.
Once defined, this standard system will remain fixed throughout time, and will become 
a feature of LSST photometry.
Observed magnitudes can be transformed to
this standard system if the shape of the SED is known, or at least
approximately transformed if colors of the target are known.

LSST photometric calibration is then separated into three parts that
address different science requirement specifications:
\begin{itemize}
\item Relative calibration: normalization of internal (instrumental) measurements in a given bandpass relative to all
other measurements made in the same bandpass across the sky. 
\item Absolute calibration of colors: determination of the five unique differences between flux normalizations of the six bands (color zero points).
\item Absolute calibration of flux: definition of the overall physical
scale of the LSST magnitude system, i.e., normalization to $F_{AB}$ in
\autoref{eqn:stdmag}. 
\end{itemize}

\iffalse
This can be made numerically explicit by writing the relation between measured magnitudes and true magnitudes 
in a linear decomposition (valid in the limit of small errors),
\begin{equation}
\label{photoSysErr}
  m_b^{std,meas} = m_b^{std,true} + \sigma + \delta_b(x,y,\alpha,\delta,t,\phi,SED) + \Delta_b.
\end{equation}
The $\sigma$ are random photometric errors (e.g., photon shot noise)
with net zero values after subtraction of known means, and the
$\Delta_b$ are unknown offsets of the zero-points of the six
photometric bands from the $F_{AB}$ normalization
(\autoref{eqn:ABmag}).  The $\delta_b$ are systematic errors of the
internal zeropoint error around $\Delta_b$ that depend on position in
the field of view ($x,y$), position on the sky ($\alpha, \delta$),
date and time, the observational bandpass ($\phi$), and the source
SED.  The average of $\delta_b$ over the survey is zero by
construction, but a value must be determined for each source location
in each image of the survey.

%We now describe how each of the three aspects of photometric
%calibration, as outlined above, will be accomplished.
\fi  

\subsubsection{Relative Calibration}

\iffalse
The greatest challenge in calibration of LSST photometry is to minimize the relative errors $\delta_b$ in
data taken throughout the 10-year multi-epoch all-sky survey.
For clarity here the six instrumental zero point offsets $\Delta_b$ are temporarily set aside (i.e. taken to be zero).
A schematic of the flow of the DR calibration measurement is shown in \autoref{Fig:DRflow}.

\begin{figure}[hbt]
\begin{center}
\includegraphics[width=1.0\hsize,clip=true]{design/figs/Calibration_Pipeline_Flowchart_DR.png}
\caption{Schematic flowchart of the LSST Data Release calibration pipelines.}
\label{Fig:DRflow}
\end{center}
\end{figure}
\fi

Precision relative calibration of LSST photometry will be accomplished by analysis of the repeated
observations of order $10^8$ selected bright ($17 < r < 20$) isolated stars during science operations of the survey.
The LSST image processing pipelines will extract raw ADU counts for these stars from each image,
and the data release Calibration Pipeline will process data from the calibration auxiliary subsystems to determine
the optical bandpass appropriate for each image.
These measurements will be used to determine calibrations for all sources detected on each image.

\iffalse
All images in the accumulated survey will first be analyzed with the Detection and Instrument Signature Removal pipelines that
detect celestial sources and assign instrumental flux values $F_b^{meas}$ (\autoref{eqn:Fo}) to each source.
This process includes corrections for cross talk, electronic bias, and subtraction of backgrounds after flat-fielding.
A calibration Reference Catalog of non-variable main sequence stars will be selected from the accumulated
Object Catalog based on their morphologies and colors.
These stars will have magnitudes $17<r<22$ to assure that measurements of their fluxes are not saturated or limited by photon counting statistics. 
These stars will be further selected to be free of overlap with other sources in order to minimize errors in assignment of ADU counts to their flux.
There will be $\sim 10^{8}$ such stars in the Reference Catalog.
These will be spaced by approximately one arc-minute on the sky, with $\sim$ 200 detected on each $14'\times14'$ CCD (at the galactic pole).
Each of these stars will eventually be observed 100-200 times in each of the six LSST filter bands. 
The Calibration Pipeline will also use data taken with the auxiliary
calibration subsystems for determination of the atmospheric absorption
model and the flat field, data from individual science images, and
accumulated data in the Object Catalog to determine $S_b^{atm}$ and
$S_b^{sys}$ for each image.
\fi

After reduction of each image in the accumulated survey,
the Calibration Pipeline will execute a global self-calibration
procedure that will seek to minimize the dispersion of the errors
in all observations of all reference stars.  This process is based on
techniques used in previous imaging surveys \citep{Gla++94, Mac++04},
and the specific implementation used by LSST will be 
based on the ``\"Ubercal'' procedure developed for SDSS
\citep{Pad++08}.  ``Calibration patches'' of order the size of a
single CCD will be defined on the camera focal plane.  
%The optimum
%size for these patches will be determined by simulation and analysis
%of precursor data, but will naturally be similar to a CCD footprint.
%So there will be $\sim$ 200-400 calibration patches, and each star $i$
%on each image $j$ will be assigned to a patch $p$.  
The LSST survey will ``dither'' pointings from epoch to epoch to
control systematic errors, so stars will fall on different patches on
different epochs across the sky.  The measured magnitudes of reference
%%stars will be transformed (\autoref{eqn:dmStar}) to the LSST standard
stars will be transformed to the LSST standard
bandpass using the accumulated estimates of the colors of each star
and the corresponding measured observational bandpasses.  The
Calibration Pipeline will minimize the relative error $\delta_b(p,j)$
in the photometric zero-point for each patch $p$ on each image $j$ of
the accumulated survey by minimizing,
\begin{equation}
\label{eqn:uberchisq}
\chi^{2} = \sum_{(i,j)} {\frac{\left( m_b^{std,meas}(i,j) - \left( m_b^{std,true}(i) + \delta_b(p,j) \right) \right)^2}
                                           {\left( \delta m_b^{std,meas}(i,j) \right)^2}}, 
\end{equation} 
where the magnitudes are in the standard system, and the summation is over all stars $i$ in all images $j$.
%The fitted parameters are the best estimates of the true in-band magnitudes of each reference star $m_b^{std,true}$
%and the zero points $\delta_b(p,j)$.
These $\delta_b(p,j)$ will be used to correct the photometry for all other sources in patch $p$ on image $j$.

%In the formulation of \autoref{eqn:uberchisq} the patch index
%represents a spatial coordinate and the image index represents a
%temporal coordinate.  There will be $\sim 10^{8}$ values of
%$m_b^{std,true}$ and $\sim 2 \times 10^{8}$ $\delta_b(p,j)$ per
%band\footnote{I.e. 200-400 patches per image $\times$ 4000 images per
%epoch $\times$ 100-200 epochs per band.} to be determined in the
%accumulated survey, and there will be $\sim 10^{10}$ measurements of
%main sequence stars per band to constrain the fitted parameters.  It
%remains to determine what computational technique works best to
%minimize this function.

\subsubsection {Absolute Calibration} 
\label{Sec:Deltam}

There are six numbers $\Delta_b$ for the entire survey that set the zeropoints of
the standard bandpasses for the six filters, i.e., that put the photometry on an AB system
(\autoref{eqn:ABmag}).  
%The global relative calibration minimizes the dispersion of
%measurement errors, but it does not address and in fact may introduce,
%systematic offsets $\Delta_b$ of the calibration scale from the
%$F_{AB}$ normalization defined in \autoref{eqn:ABmag}.  
These six numbers can be expressed in terms of a single fiducial band,
which we take to be the $r$ band,
\begin{equation}
             \Delta_b = \Delta_r + \Delta_{br}.
\end{equation}
%Any of the other bands could be chosen as the fiducial, but the LSST
%survey includes as many or more $r$ band exposures as any other band.
%With this distinction, the SRD design requirement for $\Delta_{br}$ is
%5 millimag and is 10 millimag for $\Delta_r$.

The LSST strategy to measure the observational bandpass for each
source is designed to reduce errors $\Delta_{br}$ in the five color
zero points, to meet specifications in the survey requirements.  This
process will be validated with the measured flux from 
one or more celestial sources whose physics and chemistry are believed
to be well understood, most likely hot white dwarfs whose simple
atmospheres are reasonably well-understood.
\iffalse
In principle, a single object with known
colors would be sufficient.  Hot hydrogen and helium white dwarf stars
have simple atmospheres that are reasonably well understood (model
colors are currently reliable to about 0.01 mag).  An example of a
strong sequence of HeWD in color-color space is shown in
\autoref{Fig:WDmodels}.  Catalogs of Southern WD stars have been
constructed, and a ``white dwarf calibration system'' has been
developed \citep{H+B06}.  Several WDs have been very precisely
calibrated with HST STIS measurements \citep{B+G04}.  The HST
standards will saturate normal LSST exposures, but at least one
(GD153) can be targeted with extremely short ($<$ 1 sec) exposures
under certain conditions.  It may be possible to obtain similar HST
measurements of one or more targets for use by surveys in the Southern
hemisphere.

\begin{figure}[hbt]
\begin{center}
\includegraphics[width=0.85\hsize,clip=true
%,viewport = 0 250 600 750
]{design/figs/WDmodels.pdf}
\caption{The {\it g-r} vs. {\it u-g} color-color diagram for non-variable sources from SDSS Stripe 82.
Also shown are Bergeron models for H WDs (red dashed curves) and He WDs (blue solid curves).
Different models are parametrized by log(g) (6,7,8,9,10).
The models for He WDs collapse into a single sequence for -0.25$<${\it g-r}$<$0.}
\label{Fig:WDmodels}
\end{center}
\end{figure}

Though the calibration of the LSST color scale may be done with a
small number of objects, larger sets of statistically identical
targets will be used to limit potential sources of systematic error in
the measured $\Delta_{br}$.  Systematic spatial variations and the
effects of galactic extinction on calibration measurements are sources
that are of particular importance.  Features in color-color diagrams,
such as the position of the main stellar locus, are reasonably well
understood, and have been used with success in previous surveys
\citep{Mac++04, Ive++07}.  Initial rough calibrations might
be done entirely with the main sequence locus, and ultimately this can
be used to determine the effects of galactic extinction on calibration
standards \citep{Sal++09, High09}.
\fi

At least one external flux standard will be required to determine
$\Delta_r$ (one number for the whole survey!).  While one celestial
standard would be formally sufficient, choosing a number of such
standards would provide a powerful test for $\Delta_r$.
Identification of such a standard, or set of standards, has not yet
been done.


\iffalse
\subsection{Photometric System}

The LSST will use optical filters in the camera to define six
photometric bands $b=ugrizy$ similar to the SDSS bands
\citep{Fuk++96}, as we discussed in \autoref{sec:design:filters}.
%  Nominal instrumental bandpasses computed for these
%filters with the LSST design instrumental response are shown in
%\autoref{fig:design:filters}.

%\begin{figure}[hbt]
%\begin{center}
%\includegraphics[width=1.0\hsize,clip]{design/figs/LSST_Bandpasses_1089.png}
%\caption{Nominal LSST instrumental $ugrizy$ bandpasses.  The curves are computed for the design system response of the 
%telescope, camera, and filters. }
%\label{Fig:LSSTbands}
%\end{center}
%\end{figure}
The LSST approach of directly measuring $S_b^{meas}$ will provide a
well-defined optical bandpass for each observation.  Some science
analyses may be best done by using individual ($m_b^{meas},
\phi_b^{meas}$) pairs for each detected source in each image.
But many Spectral Energy Distributions (SED) vary substantially across
the bandpass of the optical system, so even with a well-defined
bandpass it is not possible to unambiguously interpret the measured
flux unless the shape of the SED is also known.  It is desirable to
assign a single magnitude to each object in the Object Catalog in a
fashion that minimizes this uncertainty.  The LSST database will
provide access to all source detections (i.e., individual exposures)
of each object so no information is lost in making this assignment.

An LSST ``standard'' bandpass $\phi_b^{std}(\lambda)$ will be defined
as the suitably weighted mean over exposures and across the focal
plane, of the $\phi_b^{meas}$ encountered during the commissioning
(and perhaps first observing runs) of the LSST observatory.
An example of a plausible standard bandpass is shown in
\autoref{Fig:phiChange}.
Observed magnitudes can be transformed to
this standard system if the shape of the SED is known, or at least
approximately transformed if colors of the target are known.
The difference between a magnitude computed with a measured
$\phi_b^{meas}$ and that same magnitude transformed to $\phi_b^{std}$
is,
\begin{equation}
\label{eqn:dmStar}
  m_b^{std,meas} - m_b^{meas} \equiv  \Delta m_b^{std} = 2.5\,\log\left(\frac{\int_0^\infty 
f_\nu(\lambda) \phi_b^{meas}(\lambda) d\lambda} {\int_0^\infty f_\nu(\lambda) 
\phi_b^{std}(\lambda) d\lambda} \right).
\end{equation}
The source SED $f_\nu(\lambda)$ is defined by
\begin{equation}
                 F_\nu(\lambda) = F_0 f_\nu(\lambda),
\end{equation}
with $f_\nu(\lambda_b)=1$ at some chosen reference wavelength.
The value of $\lambda_b$ is entirely arbitrary, but a natural choice for this reference value is the 
mean wavelength of the normalized standard bandpass $\phi_b^{std}$.

\begin{figure}[hbt]
\begin{center}
\includegraphics[width=0.5\hsize,clip]{design/figs/phi2_0.pdf}
\vskip -0.5in
\caption{A plausible standard $\phi_b^{std}(\lambda)$ (solid lines)
defined by the 1976 U.S. Standard Atmosphere at standard temperature
and pressure viewed through an airmass $X = 1.2$ from the elevation of
Cerro Pach\'on.  The instrumental throughput is taken from the LSST
Preliminary baseline design.  Also shown is the bandpass
$\phi_b(\lambda)$ through 2 airmasses of the same atmospheric mix
(dotted lines).  Note that these curves are normalized to unity,
following \autoref{eq:design:PhiDef}. 
The atmospheric transmissivity for airmass $X=1.2$
(the standard value) and $X=2$ are shown by the dot-dashed lines
(arbitrarily normalized).}
\label{Fig:phiChange}
\end{center}
\end{figure}

\iffalse
Even in the absence of perfect knowledge of the source SED, the
transformation in \autoref{eqn:dmStar} will be exact in instances when
the actual observing conditions correspond to $\phi_b^{std}$.  Errors
from lack of knowledge of the SED will grow with the difference
between actual conditions of a given observation and the standard
bandpass.  The definition of $\phi_b^{std}$ in terms of experimentally
observed bandpasses will minimize ambiguity of LSST photometry, and
even if not totally rigorous, a way of standardizing exported LSST
magnitudes of celestial objects.
\fi

To understand the sensitivity of the photometry to the assumed SED, 
%The full SEDs of many objects will not be known, but an approximate color transformation can be used that
%will often deliver reasonably good accuracy. As a guide, 
consider the cases of the standard $\phi_b^{std}$ and observational $\phi_b$ shown in \autoref{Fig:phiChange}.
Shown in \autoref{Fig:dmStar} are transformations of observations of stars with plausible SEDs
made through this observational bandpass to $\phi_b^{std}$ as a
function of their $g-i$ color.  The small slope of the error versus color implies that even
color measurements accurate to 0.1 mag (10\%) will deliver standard magnitudes with good accuracy.

%\begin{figure}[hbt]
\begin{figure}
\begin{center}
%\includegraphics[width=0.75\hsize,clip=true]{design/figs/dmStar.pdf}
\includegraphics[width=0.5\linewidth]{design/figs/dmStar.jpg}
%\vskip -0.5in
\caption{Example photometric transformations (see \autoref{eqn:dmStar})
for Kurucz stellar models (triangles) and a power-law SED (squares). 
The vertical scale is the difference between the instrumental
magnitude and the magnitude in a plausible LSST standard photometric
system.   The horizontal axis is the color (in the instrumental
system) of a variety of stellar models. 
The Kurucz
models for $log(g)=4.0$ and two values of metallicity ($[Fe/H]=-1.5$ and 
$[Fe/H]=-0.5$) are shown as a function of effective temperature ($g-i\sim0$
for an $\sim$10,000 K A-type star, and $g-i\sim2$ for an $\sim$3000 K M0-type star). 
The power-law SEDs ($F_\nu \propto \lambda^\alpha$) are evaluated for $\alpha=(-1.5,
-1.0,-0.5,0.0,0.5,1.0)$. The observing conditions used for this calculation are described in the text and
the $\phi_b(\lambda)$ are compared in \autoref{Fig:phiChange}.}
\label{Fig:dmStar}
\end{center}
\end{figure}
\fi

%\begin{thebibliography}{}

%\bibitem[Bohlin and Gilliland 2004]{bohl04} Bohlin and Gilliland AJ, 128, 3053 (2004)
%\bibitem[Burke 2008]{burke08} Burke, D., et al., LSST Document 5367, publication in preparation (2008)
%\bibitem[Fukugita 1996]{fukugita96} Fukugita, M. et al., AJ, 111, 1748 (1996)
%\bibitem[Glazebrook 1994]{glazebrook94} Glazebrook K.,Peacock J.A., Collins, and Miller, L., MNRAS 266, 65 (1994)
%\bibitem[High 2009]{high09} High, F.W., et al., astro-ph/0903.5302, submitted to AJ (2009)
%\bibitem[Holdberg 2006]{hold06} Holdberg, J. B. and Bergeron, P, AJ 132, 1221 (2006)
%\bibitem[LSST-4169]{lsstdoc4169} Ivezic, Z, et al., LSST Document 4169 (2007)
%\bibitem[Ivezic 2007]{ivezic07b} Ivezic, Z, et al., AJ 134, 973 (2007)
%%%\bibitem[Keller 2007]{keller07} Keller, S. C., et al., astro-ph/0702511 (2007)
%\bibitem[MacDonald 2004]{macdonald04} MacDonald, E.C., et al., MNRAS 352, 1255 (2004)
%%%\bibitem[Manfroid 1996]{manfroid96} Manfroid, J., A\&AS 118, 391 (1996)
%%%\bibitem[Magnier and Cuillandre 2004]{magnier04} Magnier, E.A. and Cuillandre, J.-C., PASP 116, 449 (2004)
%%%\bibitem[Oke and Gunn 1983]{okegunn83} Oke, J. B. and Gunn, J. L. ApJ 266, 713 (1983)
%\bibitem[Padmanabhan 2008]{padman08} Padmanbhan, N, et al., ApJ 674, 1217(2008)
%\bibitem[Sale 2009]{sale09} Sale, S.E., et al., MNRAS, 392, 497 (2009)
%\bibitem[Stubbs and Tonry 2006]{sandt06} Stubbs, Christopher W. and Tonry, John L., ApJ, 646, 1436 (2006) 
%\bibitem[Stubbs 2006]{stubbs06} Stubbs, C, et al., AAS 207th Abstract 180.09 (2006)

%\end{thebibliography}



%\end{document}



\section{Astrometric Calibration}
\label{sec:design:calsimAstro}

{\it David Monet, David Burke, Tim Axelrod, R. Lynne Jones, \v Zeljko Ivezi\'c}

The astrometric calibration of LSST data is critical for many aspects
of LSST operations (pointing, assessment of camera stability, etc.)
and scientific results ranging from the measurement of stellar
parallaxes and proper motions to proper performance of difference image
analysis. 
%Fortunately, there are many different algorithms that can be
%used, and LSST will take advantage of the heritage in astrometric
%image processing developed for Pan-STARRS and SkyMapper.

The core of the astrometric algorithm is the simultaneous solution for
two types of unknowns, the coefficients that transform the coordinates
on the focal plane measured in a given exposure into some common
coordinate system (absolute astrometry), and the 
positions and motions of each star (relative astrometry).  Whereas a
direct solution exists, 
it involves the inversion of relatively large matrices and is rarely
used. Instead, the solution is based on an iterative improvement given
the prior knowledge of positions of a relatively small number of stars
(from a reference catalog or 
similar). All observations for all stars in a small area
of sky are extracted from the database. Using the catalog positions
for the stars as a first guess, the transformations from each
observation to the catalog system are computed, and then all measures
for each star are used to compute the new values for position and
motion. 

%It is important to remember the distinction between relative
%astrometry (measurement of images and the relative positions of stars
%on them) and absolute astrometry (mapping the focal plane into the
%system of right ascension and declination).

\subsection{ Absolute Astrometry} 

The current realization of the International Celestial References
Frame (ICRF) is defined by the stars in ESA's Hipparcos mission
catalog.  ESA's Gaia mission, set to launch in 2012, will improve the
ICRS and ICRF by another two orders of magnitude down to the level of
a few micro-arcseconds.

Absolute calibration consists of computing the positions of all the
detected sources and objects in the LSST imaging with respect to the
ICRF.  Were no improved catalogs available between now and LSST
commissioning, the reference catalogs would be the US Naval
Observatory's UCAC-3 catalog for bright optical stars (down to about
16th magnitude, uncomfortably close to LSST's saturation limit) or the
NASA 2MASS catalog whose near-IR positions for optical stars have an
accuracy of 70-100 milli-arcseconds (mas) for individual stars and
systematic errors in the range of 10-20 mas.  There are large numbers
of 2MASS stars in each and every LSST field of view, so the
astrometric calibration is little more than the computation of a
polynomial that maps position on the focal plane into the system of
right ascension and declination defined by the measured positions of
catalog objects.
%This 
%task is delegated to the Nightly Processing Pipeline because it is critical
%to many other data processing tasks, and it is so well understood that it can
%be executed with little, if any, human intervention.  
The transformation is
encapsulated in the World Coordinate System (WCS) keywords in the FITS header
for each image.

\iffalse
Mapping from the internal LSST coordinate system into the system of right ascension 
and declination defined by the International Celestial Reference Frame (ICRF) 
will be done by traditional Block Adjustment, and there are at least two ways to 
proceed with this technique. The mapping from each LSST frame into a reference 
catalog can be computed, and the ensemble of solutions combined using Block Adjustment.  
A second approach is to use the optical counterparts to the radio objects that define 
the ICRF to build a catalog in sequential steps of frame-to-frame overlap.

The European Space Agency's Gaia mission is scheduled to launch in December 2011, 
and it is reasonable to expect a Gaia-based astrometric catalog to be available 
by the time LSST has its First Light.  Hence, the baseline for the LSST astrometric 
calibration is the assumption that a Gaia catalog will be available. Between now 
and when this catalog appears, LSST can use existing high accuracy catalogs 
(Hipparcos, Tycho-2, UCAC) and deep catalogs (GSC-2, USNO-B1.0) for software 
development and mission planning. Experience gained from these precursor surveys 
will guide development of the algorithm for LSST.

\subsubsection{World Coordinate System and LSST FITS Files }

A World Coordinate System (WCS) transformation will be provided in the
FITS file header for all raw and derived images. 
\fi
One of the key
astrometric challenges in generating and using these WCS solutions is
the distinction between ``observed" and ``catalog" coordinates.  When
LSST takes an image, the stars and galaxies are at their observed
positions.  These positions include the astrometric effects of proper
motion, parallax, differential refraction, differential aberration,
and others.  Most applications work in catalog coordinates such as the
J2000 positions for objects or the equivalent for image
manipulation. The astrometric calibration will provide a rigorous
method for going between these coordinate systems.


\subsection{ Differential Astrometry }

Differential astrometry is for most science the more important job to
be done. The differential
solution, which provides measures for the stellar parallax, proper
motion, and perturbations (e.g., due to binary companions), can be
substantially more accurate than the 
knowledge of the absolute coordinates of an object. The task is to
measure centroids on images and to compute the transformation from the
current frame into the mean coordinate system of other LSST data, such
as the deep image stacks or the different images from the multi-epoch
data set.  The photon noise limit in determining the position of the
centroiding of a star is roughly half the FWHM of the seeing disk,
divided by the signal-to-noise ratio of the detection of the star. 
The expectation is that atmospheric seeing will be the
dominant source of astrometric error for sources not dominated by
photon statistics.  Experiments with wide-field imaging on the Subaru
Telescope (\autoref{sec:com:PMacc}) suggest that
accuracy will be better than 10 mas per exposure in the
baseline LSST cadence, although it may be worse with objects with
unusual SEDs such that simple differential color
refraction analysis fails, or for exposures taken at extreme zenith
angles. 

Perhaps the biggest unknown in discussion of differential astrometry
is the size of the ``patch" on the sky over which the astrometric
solution is taken. If the patch is small enough, the astrometric
impact of the unaveraged turbulence can be mapped with a simple
polynomial, and the differential astrometric accuracy approaches that
set by the photon statistics.  Our current understanding of
atmospheric turbulence suggests that we will be able to work with
patches between a few and 10 arcmin in size, small enough that the
geometry can fit with low-order spatial polynomials.  The current
approach is to use the 
JPL HEALPix tessellation strategy. 
% with the number of sides being left as
%a free parameter until the LSST site conditions have been characterized.
%For software development purposes, a solution side of 256 gives HEALPix
%of approximately 14 arcminutes on a side.  
For each solution HEALPix(el),
separate spatial transformations are computed for each CCD of each
observation.  These produce measures for each object in a mean coordinate
system, and these measures can be fit for position, proper motion, parallax,
refraction, perturbations from unseen companions, and other astrometric
signals.  Given
the very faint limiting magnitude of LSST, there should be 
be a sufficient number of astrometrically useful galaxies to deliver a
reasonable zero-point within each HEALpix\footnote{Quasars will be
  less useful; they are less numerous, and their very different SEDs
  cause different refraction from stars.}. The characterization of the
zero-point errors and the astrometric utility of galaxies will be the
major work area for the astrometric calibration team.

\iffalse
To estimate the
complexity of the differential astrometric 
solution, a strategy based on the HEALPix tessellation scheme was
evaluated. LSST is expected to take 300,000 exposures per year which
means that 30,000,000 tile solutions per year are to be expected. With
appropriate optimization of database organization and computing
techniques it should be possible to carry out all-sky astrometric
solutions several times per year. This will benefit a number of
scientific investigations.

A critical aspect of the LSST differential astrometric solution
algorithm is its ability to tie the zero points of the parallax and
proper motion solutions in each patch to the external zero points
defined by galaxies and other extremely distant objects.  Studies into
the astrometric accuracy (\autoref{sec:com:PMacc}) and solution patch
size (simulations 
as well as results from Pan-STARRS and SkyMapper) will be merged with
expectations for the number, brightness, and shape of galaxies to
produce more robust algorithms, particularly as a function of Galactic
latitude, as well as predictions for the zero point uncertainties.
These predictions will become more reliable as further studies of
the seeing at the proposed LSST site become available, and as the
Pan-STARRS and SkyMapper surveys collect data over a wide range of
atmospheric conditions.

The expected accuracy of trigonometric parallax and proper motion 
measurements is discussed in \autoref{sec:com:PMacc}.
\fi


==> galaxies/alignments.tex <==
% ======================================================================
%+
% NAME:
%   galaxies/alignments.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================

\subsection{Intrinsic Alignments}



==> galaxies/bridge.tex <==

Observations and hierachical models of structure formation suggest that
gravitational interactions and mergers between galaxies are important aspects of
galactic evolution.  Mergers can significantly alter a galaxy's morphology,
luminosity, color, size, star formation rate (SFR), and mass distribution  over
a relatively short timescale.  However, quantifying the role merging plays in
galaxy evolution and mass build-up has been challenging, mostly because (gas
rich) mergers involve physics (e.g., feedback from supernovae and AGN) which are
difficult to model, and samples that span a large range in luminosity and
redshift space have been difficult to assemble in an unbiased manner.

In a $\lambda$CMD model the rate that dark matter halos merge together is one of
the fundamental processes in structure formation.  Semi-analytical models and
N-body simulations predict that the rate at which dark matter halos merge evolves with
redshift as $(1+z)^{m}$, with 1.0<m>3.5 (Gottlober et al, 2001; Berrier et al.
2006; Fakhouri \& Ma 2008).  It is difficult to directly compare the dark matter
halo merger rate with the galaxy merger rate due to the uncertainty in the halo
occupation number, however measuring the frequency that galaxies merge as a
function of cosmic epoch can place powerful constraints on the models of
structure formation in the Universe.

The galaxy merger rate is traditionally estimated by measuring the frequency of
galaxies residing in close pairs, or those with morphological distortions
typically associated with interactions (e.g., tidal tails, stellar bridges,
etc.).  The detection of distortions is done either by visual analysis and
classification (e.g., Le Fevre et al. 2000; Bridge et al.  2009) or through the
use of more general structural parameters, such as asymmetry or concentration
(e.g., Abraham et al. 1996; Conselice et al. 2003; Lotz et al. 2008).  Within the
past two decades numerous observational studies have been focused on measuring
the merger rate, yielding highly discrepant values of ``m", ranging from no
evolution ($m \sim 0$) to strong evolution ($m \sim  5$) (Zepf \& Koo 1989;
Carlberg 1994,2000; Patton et al. 2000; 2002; Bundy et al. 2004; Lin et al.
2004; Bridge et al. 2007,2009; Lotz et al.2008).  This discrepancy stems largely
from small sample sizes, of only a few ten's to a hundred of mergers or close
pairs, improperly accounting for the timescales over which different techniques
are sensitive, or the difficulty in tying together surveys at high and low
redshift.

Despite the existence of many large scale surveys, such as SDSS, COSMOS, and the
CFHTLS-Deep and Wide, a clear measure of the merger rate evolution remains
elusive.  Downsizing argues that at low redshifts the majority of star formation
is occurring in lower mass galaxies ($ < 10^{10}$ rm$_\odot$).  SDSS suffers from
incompleteness at stellar masses $< 10^{10}$ M$_\odot$ for $z < 0.15$ due to sensitivity
limits.  While the CFHTLS-DEEP and COSMOS surveys can detect low-z, low mass
galaxies, the volumes are too small to contain large numbers of these galaxies.
LSST will have both the depth and volume to detect a large number of the low
mass galaxies responsible for much of the star formation at low redshift.

Wide area surveys like the SDSS identify large numbers of close pairs, but lack
the depth to probe L* galaxies at redshifts beyond a redshift of about $z =
0.1$.  Surveys like COSMOS and CFHTLS-Deep can derive good statistics on the
merger rate from morphologies and pair counts between $0.4 < z < 1$ for log M
(M$_\odot$) $> 10.7$, but lack the area to connect with studies at low redshift.
LSST is well matched to the depths, wavelength coverage, seeing and plate scale
($\sim 0.2$ arcsec/pixel) of the CFHTLS-Deep survey, but over an area which is a
factor of 5000 larger.  In particular, LSST will be ideal for detecting low
surface brightness features such as tidal tails and bridges which are signpost
of recent merges out to $z \sim 0.8$.  LSST will reach comparable surface
brightness limits as the CFHTLS-Deep survey (28 mag/square arcsec), and should
therefore detect on the order of 15 million galaxies undergoing a strong tidal
interaction.  It will therefore be the definitive survey to study the merger
rate in a self consistent manner from the local Universe out to $z \sim 1$.

One of the advantages of the LSST survey for studying the evolving merger rate,
is the dense sampling of parameter space.  It will be possible to explore and
quantify the incidence of mergers as a function of environment, merger stage,
stellar mass, and luminosity.  LSST's six-band photometry will result in
photometric redshift accuracies of about 0.03(1+z), which is comparable to or
better than those used in other studies for the identification of close galaxy
pairs, and allow for the selection of merging galaxies with a wide range in
color.  In particular, the ability to detect so-called ``dry mergers``, mergers
between gas-poor, early-type galaxies which have been invoked to explain the
stellar mass build-up of today's most massive ellipticals (e.g., van Dokkum
2005, Bell et al 2007) will be greatly facilitated by LSST.  Current surveys
seem to detect only about 50-70 dry-mergers per square degree for $0.1 < z <
1.0$, based on optical colors of the galaxies. With LSST, we should be able to
identify more than a million dry mergers out to $z \sim 1.0$.

The wide area coverage of LSST will be critical for addressing the effects of
cosmic variance on measures of the merger rate.  Field-to-field variance of the
merger rate has only been minimally addressed, but suggests that the merger
fraction can vary by a factor of two (Bridge et al. 2009), and the uncertainty
in ``m" can double (up to 80\%), even on projected scales of a square degree.




==> galaxies/hod.tex <==
% ======================================================================
%+
% NAME:
%   galaxies/hod.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================

%\subsection{Halo Occupations for Different Kinds of Galaxies}

%Correlation functions will be measured for galaxies tagged by
%redshift, luminosity, color, size, and morphology. Mock catalogs will
%be generated from galaxy-evolution models, and the comparison will be
%used to test the models and constrain their parameters.




==> galaxies/lotz.tex <==
Galaxy Mergers  --
{\it Science Questions:} \\
Galaxies must grow with time through both discrete galaxy mergers and smooth gas accretion.  When and how this growth occurs remains an outstanding observational question.  The smooth accretion of gas and dark matter onto distant galaxies is extremely challenging to observe,  and complex baryonic physics makes it difficult to infer a galaxy’s past assembly history.   In contrast,  counting galaxy mergers is relatively straightforward.   By comparing the frequency of galaxy mergers to the mass growth in galaxies,  one can place robust constraints on the importance of discrete galaxy mergers in galaxy assembly throughout cosmic time.  The mass accretion rate via mergers is likely to be be a strong function of galaxy mass and environment. 

In addition to contributing to the overall buildup of galaxy mass, the violent processes associated with mergers are expected to significantly influence the star-formation histories, structure, and central black hole growth of galaxies.  However, other physics mechanisms may influence galaxy evolution in similar ways, so direct observations of galaxy mergers are needed to answer the following questions:

$\bullet$ What fraction of the global star-formation density is driven by mergers and interactions?  Is the frequency of galaxy mergers consistent with the 'tightness' of the specific star-formation rate (SFR/M*) v. stellar mass relation throughout time ?

$\bullet$ Are typical red spheroids and bulges formed by major mergers, or secular evolution?  Do z>1 compact galaxies grow in size by (minor) mergers?

$\bullet$ Are today's most massive ellipticals formed via dissapationless mergers?  If so, when?

$\bullet$ Do gas-rich mergers fuel active galactic nuclei? Which forms first, the bulge or SMBH?           

{\it Why LSST?} \\
While it is not well known how frequently galaxy mergers occur,  it is known that they are hard to find. The merger of two comparable mass galaxies may take $\sim$ 1-2 Gyr to complete,  but the signatures of the merger are obvious for only a fraction of this time. Galaxies at $z<1$ with clear signatures of merger activity are relatively rare ($<$10-15\% of $\sim$ L$^*$ galaxies at $z < 1$,$<$5\% at $z=0$).  Current deep Hubble Space Telescope galaxy surveys have detected only a few thousand galaxy merger candidates at $0.2 < z < 1.2$,  and only a few hundred candidates at $z>1.2$. {\bf CFHTLS??} The full LSST survey will cover an area $\sim$ 10$^4$ these surveys, and detect at least several million galaxy mergers. 

Frustratingly, the evolution of the global merger rate with time continues to be strongly debated, despite efforts from many different groups.   No single study conducted so far has been able to uniformly map the galaxy mergers rate from $z=0$ to $z\geq 2$, as current studies must trade off between depth and volume.    Very few merger studies have been done with SDSS (optimized for the $z< 0.2$ universe), in part because fiber collisions and low precision photometric redshifts prevent accurate pairs studies, and the SDSS data-pipeline has difficulty deblending the images of nearby galaxy mergers. Deeper spectroscopic and imaging studies probe the $z \sim 0.2 - 1.$ universe,  but do not have the volume to also constrain the low redshift universe or the depth at near-infrared wavelengths to constrain the $z>1$ universe. Ultra-deep Hubble Space Telescope studies (GOODS, UDF) can detect L$^*$ mergers at 
$z > 1$,  but have very small volumes and are subject to cosmic variance effects. Nevertheless, the results of these different studies have been patched together,  and much of the inferred evolution in the galaxy merger rate is the result of the factor of $\sim$ 10 difference between the $z=0$ and higher redshift surveys.  {\bf same is true for red galaxy evolution, eg Faber et al 2007}  One worries that unknown systematic effects between the low and higher redshift surveys are biasing these results.  Unlike these current studies,  LSST has the depth, volume, and wavelength coverage needed to perform a uniform study of L$^*$ mergers out to z~2.  
            
The large number statistics and depth of the LSST dataset will be invaluable for identifying a sample of mergers large enough to explore questions beyond simply counting the number of mergers.  A large number of merger parameters -- galaxy masses and mass ratio, gas fractions, environment --  are important to understanding the role of mergers in galaxy evolution.   Gas-rich mergers may contribute significantly to formation of stars at early times,  while gas-poor mergers may be the only way to form today's most massive elliptical galaxies.    Major mergers could scramble disks, form bulges, and fuel super-massive black holes,  while minor mergers could grow the stellar halos and outer disks of massive galaxies.    The tidal debris produced by galaxy interactions could become the intercluster light and gas in very dense environments,  or fall back onto the merger remnants and reform star-forming disks in less extreme locations.     Probing these different kinds of mergers, as a function of redshift, mass, and environment,  requires large number statistics. 
           
Finally, the cadence of the LSST observations will open several exciting new avenues.   It will be possible to identify optically variable AGN in mergers and constrain the SMBH growth as a function of merger stage, mass, and redshift.   With millions of galaxy mergers with high star-formation rates,  we will detect a significant number of supernovae over the 10 year LSST survey.   We will be able to determine the rate of SN I, II in mergers, and obtain independent constraints on the merger star-formation rates and initial stellar mass functions.  

{\it Methodology:}\\

LSST galaxy mergers may be identified by \\

     (1) short-lived strong morphological disturbances, such as strong asymmetries and double nuclei, which occur during the close encounters and final merger stages and are  apparent for only a few 100 Myr. These will be most easily found in lower $z$ ($<$ 0.2) galaxies, where the LSST 0.7\arcsec spatial resolutions corresponds to 1-2 kpc.  {\bf mention lopsidedness?  require similar spatial resolution}

     (2) the statistical excess of galaxy pairs with projected separations small enough such that they has a high probability of merging within a few 100 Myr.  With ~0.7\arcsec PSF,  galaxies with projected separations $>$ 10 kpc (2x PSF) will be detectable to z $\sim$ 5.   With LSST's high quality photometric redshifts and large number statistics,  it will be possible to accurately measure the galaxy pair fraction to high precision (although the identification of any given pair will be uncertain).  {\bf possible with CFHTLS but I don't know of any existing studies}

      (3) longer-lived but lower surface brightness extended tidal tails,  which occur for $\sim$ 0.5 Gyr after the initial encounter and for up to 1 Gyr after the merger event.   These tails are the longest-lived merger signatures for gas-rich major mergers, and should be easily detected at $z \sim$ 1 in the full depth LSST r-i-z images (see Figure xx).  {\bf mention development of automated tidal tail detector?} 

      (4) residual fine structures (faint asymmetries, shells, and dust features) detected in smooth-model subtracted images.  These post-merger residual structures are most visible for gas-rich merger remnants, and contribute $<$ 1-5\% of the total galaxy light, with surface brightnesses $\sim$ 28 mag per arcsec. {\bf show Van Dokkum 2005 images?}

Each of these approaches will yield independent estimates of the merger rate as a function of redshift, stellar mass, and environment. 
However, each technique probes different stages of the merger process, and is sensitive to different merger parameters, therefore the comparison of the different 'merger' samples can constrain how the merger sequence and parameter spaces are populated.   For example,  all mergers will go through close pair and double nuclei stages,  but only gas-rich major mergers will have long tidal tails visible in LSST at $z \sim 1$.     

==> galaxies/ls_environ.tex <==
% ======================================================================
%+
% NAME:
%   galaxies/ls_environ.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================

\subsection{Large-scale Environment} \label{sec:gal:ls_environment}

\noindent{\it J. Newman} % (Writing team)

LSST measurements of large-scale structure and weak lensing will
provide maps of over- and under-densities. These will generally be on
large scales, while galaxy evolution is thought to depend on
densities on more local scales. However, there are second-order
effects (e.g. halo assembly bias) that could have an influence on
galaxy formation. The large LSST database will allow us to study the
trends of luminosity function, colors, and morphology with large
scale environment.



==> galaxies/voids.tex <==
% ======================================================================
%+
% NAME:
%   galaxies/voids.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
\subsection{Galaxies in Voids}
\noindent{\it Harry C. Ferguson} % (Writing team)

One of the best ways to test whether galaxy evolution is regulated by
internal or external processes is to compare galaxies in very
low-density regions (voids) to those in high-density regions. Existing
studies indicate that the differences between void galaxies and those
on the walls of voids are subtle, but qualitatively consistent with
the expectations from semi-analytic models. Galaxies in voids tend
to be bluer and of later morphological type than those in denser
regions.  Nonetheless, the observations suggest that the individual halos 
within voids are populated by about the same number of galaxies at fixed
mass as halos in higher density regions \citep{2008ApJ...686...53T}.
The statistics are still relatively sparse and limited mostly to
luminous galaxies. SDSS provides $\sim 10^3$ void 
galaxies within $z<0.089$ \citep{2004ApJ...617...50R}. Roughly 7\% of galaxies
are found in voids with $\delta \rho/ \rho < -0.6$.  

Voids will be seen at very low contrast in the LSST photometric redshift
data. Initial studies using only LSST can stack photometrically selected
voids and study the luminosity function, colors, incidence of mergers,
and trends with redshift for galaxies in the voids compared to denser
regions. Followup studies with spectroscopy can better delineate the
voids and study the stellar populations, incidence of AGN and emission-line
properties of the void galaxies in more detail.


==> lss/cross/cross.tex <==
% ======================================================================
%+
% NAME:
%   lss/cross/cross.tex
%
% PURPOSE: 
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS: Jeff Newman (jeffrey.a.newman@gmail.com)
%	   Tony Tyson 
%
%-
% ======================================================================
\section{Photometric Redshift Error Distribution} \label{sec:lss:cross}

{\it Jeff Newman and Tony Tyson}

Although the auto-correlation - the clustering of a sample with itself
- contains a great deal of information, interpreting angular auto-correlations
is critically dependent upon understanding the redshift distribution
of the sample (via Limber's equation). With LSST, we can use
photometric redshifts to determine these redshift distributions, but
only as well as we understand the photo-z's. 

Cross-correlations - the clustering of a sample with another sample -
provide additional information, both on clustering statistics
(e.g. the cross-correlation of red or blue galaxies vs. galaxy
clusters helps us to constrain the effects of environment on galaxy
properties) and on redshift distributions (as the strength of the
cross-correlation depends on the overlap in redshift). LSST will
provide a variety of novel samples for such studies. Cross-correlations
between LSST objects and spectroscopic samples can be particularly
powerful, as this both greatly reduces the impact of redshift
uncertainties affecting Limber's equation, and can provide accurate
reconstruction of redshift distributions for photometric samples with
readily feasible spectroscopic samples \citep{newman08}. Using these
techniques, root-mean-square errors in recovering both the mean
redshift and the $\sigma$ of the redshift distribution for a single
photometric redshift bin with true distribution given by a Gaussian
are $1.4\times 10^{-3}({\sigma_z/0.1})({\Sigma_p/10})^{-0.3}({dN_s/dz
/ 25,000 })^{-1/2}$, where $\sigma_z$ is the true Gaussian $\sigma$,
$\Sigma_p$ is the surface density of the photometric sample in
galaxies/arcmin$^2$, and $dN_s/dz$ is the number of galaxies with a
spectroscopic redshift per unit $z$.  See \autoref{sec:photoz:cross}
for more details.


Even without spectroscopic samples, cross-correlations between samples
from different photo-z bins can provide powerful constraints on
redshift distributions (or photometric redshift errors). For example,
given a Gaussian photo-z error distribution, the amplitude of the
cross-bin galaxy power spectrum decreases with the separation between
the bins in a predictable manner. If the observed cross-power spectra
do not follow the expectation, the assumed photo-z error distribution
may be wrong. Using Markov Chain Monte Carlo techniques, one can then
estimate the photo-z error distribution, along with a variety of other
parameters, from the full set of galaxy auto- and cross-power spectra.  


==> performance/performance.tex <==
% ======================================================================
%+
% NAME:
%   performance/performance.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================

\chapter[Performance]
{Anticipated and Simulated Performance of the Baseline System Design (Including Site)}
\label{chp:perform}

{\bf \v Zeljko Ivezi\'c, Chuck Claver are responsible for this chapter.}
\begin{itemize} 
  \item	Performance Models and Simulations {\bf \v Zeljko Ivezi\'c, Andy Connolly}
  \item Delivered Image Quality {\bf Chuck Claver, Jacques Sebag}
  \item	Sky Background and Instrumental Artifacts {\bf Lynne Jones,
    Chuck Claver}
  \item Methods of Photometric calibration {\bf David Burke}
  \item Methods of Astrometric calibration {\bf Dave Monet}
\end{itemize}

The motivation for the system design can be found in the paper by
\citet{Ive++08}, and in \autoref{chp:design}.


\v Zeljko thinks that this chapter should be removed (and others
have agreed, his notes show). Performance Models and Simulations is
in the next chapter, Delivered Image Quality is probably in Appendix,
Sky Background and Instrumental Artifacts should be there too, but
perhaps it is enough to have sky brightness listed in the next
chapter, and the last two should go whereever we put sections
such as DM description, etc. 



% ----------------------------------------------------------------------

\bibliographystyle{SciBook}
\bibliography{performance/performance} 

% ======================================================================


==> stronglens/sl-clusterarcstats.tex <==
% ======================================================================
%+
% NAME:
%   stronglens/sl-clusterarcstats.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
% ============================================================================

\section{ Cluster Properties and Cosmography from Arc Statistics }
\label{sec:sl:arcstats}

\noindent{\it J.~Jeee, M.~Oguri, A.~Zenntner}  % (Writing team)

The strong lensing cross-section is a very sensitive function of
cluster abundance, mass and concentration, and also a function of
cosmological parameters via the distance ratios. The very largest
Einstein radii may be a good probe of sigma8. To measure the
cross-section, one needs to count giant arcs as function of zd, zs,
dtheta, and then infer n(M,z), c(z), and cosmological parameters,
using numerically-simulated clusters to understand various projection
effects. One also needs a very good understanding of source galaxy
population - their sizes and morphologies as well as their number
counts, and also accurate photo-zs. Without any of these ingredients,
arc statistics becomes a probe of that missing ingredient: the
redshifts and sizes of the very faintest galaxies may be able to be
constrained in this way. 

% ============================================================================



==> stronglens/sl-exotica.tex <==
% ======================================================================
%+
% NAME:
%   stronglens/sl-exotica.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
% INPUTS:
%
%
% DEPENDENCIES:
%
%
% EXAMPLES:
%
%
% BUGS:
%
%
% AUTHORS:
%   Phil Marshall <pjm@physics.ucsb.edu>
%   Masamune Oguri <oguri@slac.stanford.edu>
%
%-
% ======================================================================

\section{Exotic Gravitational Lenses in the LSST Survey}
\label{sec:sl:exotica}

\noindent{\it P.~J.~Marshall, M.~Oguri}  % (Writing team)

Among the few tens of thousands of strong lenses detected by LSST,
some will show bizarre image configrations not yet seen. Galaxy disks,
mergers and binaries, and groups and clusters of galaxies will all
have complex caustic structure, with some interesting critical
points. While lens geometries close to these ``higher order
catastrophes'' are expected to be very rare, they may enable some quite
interesting applications. Since they are by definition associated with
points where the gradient and curvature of the magnification satisfy
some very particular relations, the resulting image configurations
allow accurate local measurements of density profiles and small scale
potential fluctuations. Lenses sources close to higher order
catastrophe points can also show very high magnification, making them
prime targets for cosmic telescope projects. 

% ============================================================================
% To-do list, items double-commented for easy report-compilation
%  (see header of stronglens.tex for details)
%
% % - Only initial preamble in place: needs both science justification
% %   and technical feasibility writing
% % 
% ============================================================================



==> stronglens/sl-sne.tex <==
% ======================================================================
%+
% NAME:
%   stronglens/sl-sne.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
\section{ Measuring the Physical Properties and Rates of High Redshift  SNe with a Large Array of Cosmic Telescopes }

\noindent{\it M.~Wood-Vasey, G. Dobler}  % (Writing team)

A few hundred lensed supernovae are expected to be detected by LSST,
with the numbers roughly equally split between core-collapse and type
Ia. The magnification of the lens brings distant SNe above detection
limit - with a well-characterised lens population, this should allow
SNe rates at z > 1 to be estimated. 

Microlensing by stars in the lens galaxy will affect the apparent
fluxes of the multiply-imaged SNe - but this magnification changes as
source expands, giving a new and independent probe of the photosphere
expansion rate. 

It is possible that some fraction of the supernova-like events
detected as being multiply-imaged are actually the afterglows of gamma
ray bursts. If their character can be ascertained, then study of the
burst precursor and early stages may be possible in the third or
fourth image of a quad lens system. 


==> supernovae/sn-cadencerequirements.tex <==
\section{Cadence Requirements}
\label{sec:sn:cadence} 
\noindent{\it Zeljko Ivezic, astro-ph} % (Writing team)
% ============================================================================
% MWV:  This section is pretty decent.  
%
% % - Strauss says to integrate this with Survey Requirements Chapter.  No objections.
% % - 2009/05/03 - MWV: I don't know if this has been done or not.
% ============================================================================


The physical size of a supernova explosion dictates its photometric evolution.
In the early hours of the explosions, changes are very rapid, while for the
first few months as the photosphere expands and cools, changes happen on
time scales of days.  As the supernova continues to expand, changes begin to
happen on time scales of months to years.  The LSST is perfectly poised to observe
supernovae on all these scales, with the large-aperture sensitivity required to
study supernovae across 10 magnitudes of variation\footnote{10 magnitudes being in the deep-drilling fields and also the span from the coadded stacks to the individual exposures}.

%%%%%%%%%% Begin Ivezic astro-ph text
To fully 
exploit the supernova science potential, light curves sampled in multiple
bands every few days over the course of a few months are required. This is
essential to search for systematic differences in supernova populations 
(e.g., due to progenitor channels) which 
may masquerade as cosmological effects, as well as to determine photometric 
redshifts from the supernovae themselves. Unlike other cosmological probes,
even a single object can provide useful constraints and, therefore, a large 
number of SN across the sky can enable a high angular resolution search for 
any dependence of dark energy properties on direction, which 
would be an indicator of new physics. Given the expected SN flux distribution, the 
single visit depth should be at least $r\sim24$. Good image quality is
required to separate SN photometrically from 
their host galaxies. Observations in at least five photometric bands are 
necessary to ensure that, for any given
supernova, light curves in several bands will be obtained (due to the spread in
redshift). The importance of K-corrections to supernova cosmology implies that the
calibration of the relative offsets in photometric zero points between filters and
the knowledge of the system response functions, especially near the edges of
bandpasses, must be accurate to about 1\% \citep{wood-vasey07}.  Similar
photometric accuracy is required for photometric redshifts of galaxies. Deeper data 
($r>26$) for small areas of the sky can extend the discovery of SN to a mean 
redshift of 0.7 (from $\sim0.5$ for the main survey), with some objects beyond $z\sim$1
\citep{garnavich05,pinto06}. The added statistical leverage 
on the ``pre-acceleration'' era would improve constraints on the properties of 
dark energy as a function of redshift.

\autoref{tab:sn:cadence_requirements} presents a somewhat crude listing of science topics and estimated cadence requirements.  These cadence requirements need to be more fully considered and the most demanding ones further developed and refined.

%%%%%%%%%% End Ivezic astro-ph text

\input{supernovae/tables/sn_cadence_requirements}





==> supernovae/sn-deepdrilling.tex <==
\section{Deep Drilling for \sneia}
\label{sec:sn:deepdrilling}

\noindent{\it Phil Pinto, Peter Garnavich } % (Michael Wood-Vasey)

The deeper LSST supernova sample will come from a ``deep-drilling'' mode search 
of a more limited area of sky, with longer exposure times and frequent
repeat exposures on the chosen fields. 
This specialized cadence will allow for a subset of 
1,500~\sneia/year that are well sampled and can be statistically used 
to leverage the rest of the sample.
At $z \approx 1$, \sneia are red, and fainter than can be followed in
standard single exposures reaching $r \sim 24$, but the deep drilling mode will reach $r=26$.  Assuming we can limit both 
the systematics and uncertainties due to lack of 
spectroscopic followup on the vast majority of the supernovae --
an area of intensive current research \citep[c.f.,][]{barris04,prieto06} --
the resulting redshift-distance relation data may be able to constrain models
of variable $w$ in the nearby universe ($z<1$) to better than 1\% when combined with priors from 
other experiments such as Planck.  The degeneracy line of the weak lens
technique in $w-\Om$ space is nearly orthogonal to that of
\snia-based measurements of luminosity distance versus redshift, 
making these two measurements extremely complementary.

Because the LSST surveys such a
large volume per field, and supernovae are relatively frequent events,
a relatively few
fields spaced about the sky would suffice to measure cosmological
parameters as a function of redshift and direction. 
%Such high-redshift
%supernovae are of course very red in observed bands, and are very
%faint. the LSST would thus need red sensitivity and relatively long dwell
%times, with frequent repeat revisits to chosen fields.  Because of the
%small number of fields, the overall impact on scheduling is not expected to
%be severe. 
Observations carried out over a single night to $r=26$, $z=25$
(10--20 minutes per band) are required every five days in each of four
bands (not necessarily on the same day). Individual fields would be
followed for four or five 
months to allow for complete coverage of detected
supernovae light curves (the length that a single light curve could be
followed is roughly three months at $z = 1$, but with a three-month
campaign, all supernovae that started after the first few weeks of the
period would have only partial coverage).  If we assume no evolution
in the supernova rate, 
we estimate that this survey will yield 
more than 200 high-quality supernovae in each $10^\circ$ field in a dedicated
year-long campaign. These
light curves will have unprecedented detail, with 60--100 photometric points per
light curve total in five bands. The sample will have a mean redshift of $0.7$ and
extend (with more limited color coverage) out to $z\sim1$. 
Such detailed
color information will allow fitting for photometric redshifts from the
supernovae themselves.  Realistic simulations (see \autoref{fig:sn:sn4plot}) show
that fitting multi-color light curves of the quality we hope to get
for host-galaxy reddening, redshift, and distance modulus 
simultaneously yields redshift errors of $0.7\%(1+z)$ and extinctions
accurate to $0.03$ in $A_V$. 

% Figure by Phil Pinto?  Made for LSST; likely presented in previous LSST SNSC posters.
\begin{figure}
\begin{center}
%\includegraphics[width=12cm,angle=270]{supernovae/figs/sn4plot.pdf}
\includegraphics[width=8cm,angle=270]{supernovae/figs/sn4plot.pdf}
\caption[Deep Drilling \snia Light Curve Parameters]{
Simulations showing the errors in recovering $z < 1$ SN properties from light
curves obtained in the deep-drilling mode described in
\autoref{sec:sn:deepdrilling}.
(clockwise from top left): 
(a) redshift errors; mean = $-$0.0004, $\sigma_z$=0.007. 
(b) distance modulus $\mu$ error; mean = $-$0.006, $\sigma_\mu$=0.16. 
(c) reddening error; mean = 0.002, $\sigma_{A_V}$ = 0.03.
(d) correlation between redshift and distance modulus errors. The
covariance is weak.
%[From LSST Design Reference Mission (DRM).]
}
\label{fig:sn:sn4plot}
\end{center}
\end{figure} 

The photometric redshifts of the supernovae can be compared to those of their
host galaxies, and since the area on the sky is limited, a wide-field
multiple-object-spectrograph such as a southern WFMOS could obtain
spectroscopic followup for at least 1,000 \sneia/yr in the deep drilling fields
with 15 nights of observing time while obtaining spectroscopy of all supernova
host galaxies down to $M\sim-17$ at a redshift of $z\sim1$ and $M\sim-15$ out
to a redshift of $z\sim0.5$.
%From
%supernova photometric redshifts 
%alone, and with no other priors, the first two years of such a survey can
%make independent measurements of $\Omega_M$ and $\Omega_\Lambda$ to better
%than 10\%, $w$ to 0.07, and $w'$ to 0.3 in {\em each field
%  surveyed}. 
% \autoref{fig:sn:snlc} shows a typical light-curve for a supernova
% at $z=0.8$ 
% from a complete simulation of the high-redshift supernova sample,
% incorporating a realistic observing cadence, telescope and detector
% throughput, and the uncertainties inherent in the light curve fitting
% procedure.   
%Using a randomly selected sample of 2000~\sneia  from one
%realization, Figures \ref{fig:sn:snoo}, \ref{fig:sn:snow}, and
%\ref{fig:sn:snww} show the resulting constraints on cosmological
%parameters possible in the first year of the LSST survey.  

These \sneia will serve as extended probes from the sample beyond the redshifts of 
50,000~\sneia per year sampled by the universal cadence.
Combined, these data could be used to separately constrain
the expansion rate and evolution of $w$ in different directions
in the Universe back to only a few billion years after the Big Bang.

% Figure by Phil Pinto?  Made for LSST; likely presented in previous LSST SNSC posters.
% \begin{figure}
% \begin{center}
% \includegraphics[width=0.6\linewidth,angle=0]{supernovae/figs/snlc.jpg}
% \caption[Typical LSST \snia light curve]{Typical light-curve and fit resulting from
% observation of a $z=0.8$ supernova observed with 10 minutes of exposure time
% in VRI and 20 minutes in $z$ every five days.
% %[From LSST DRM.  Figure by Phil Pinto]
% }
% \label{fig:sn:snlc}
% \end{center}
% \end{figure} 

%% Figure by Phil Pinto?  Made for LSST; likely presented in previous LSST SNSC posters.
%\begin{figure}
%\includegraphics[width=5in,angle=270]{supernovae/figs/snoo.pdf}
%\caption[\Om, \OL with subsample of \sneia]{
%One, two, and three-$\sigma$ confidence contours for
%(\Om, \OL) for 2000 supernovae to a redshift of $z=1$ from
%one realization of the simulation described in the text. No prior knowledge
%of $H_0$ is assumed, and $w$ was assumed to evolve with redshift as 
%$w = w_0 + w_1(1+z)$.
%[From LSST DRM. Figure by Phil Pinto]
%}
%\label{fig:sn:snoo}
%\end{figure}  
%% Figure by Phil Pinto?  Made for LSST; likely presented in previous LSST SNSC posters.
%\begin{figure}
%\includegraphics[width=5in,angle=270]{supernovae/figs/snow.pdf}
%\caption[\Om, $w$ with subsample of \sneia]{
%One, two, and three-$\sigma$ confidence contours for
%\Om and $w$ (here assumed constant) for the supernova sample used
%in \autoref{fig:sn:snoo}.
%No prior knowledge of $H_0$ was assumed. %, and the exact prior $w_1 = 0$.
%[From LSST DRM. Figure by Phil Pinto]
%}
%\label{fig:sn:snow}
%\end{figure} 
%\begin{figure}
%\includegraphics[width=5in,angle=270]{supernovae/figs/snww.pdf}
%\caption[$w_0,w_z$ from \sneia with LSST]{
%1, 2, and 3 $\sigma$ confidence contours for
%$(w_0, w_1)$ ($w = w_0 + w_1(1+z)$) for the supernova sample used in
%\autoref{fig:sn:snoo}.  No
%prior knowledge of $H_0$; $\Omega_{tot}=1$ was assumed.
%[From LSST DRM. Figure by Phil Pinto]
%}
%\label{fig:sn:snww} 
%\end{figure}
% MWV - 2009/04/01 : True, but maybe not appropriate for the scibook section
% Note that this program may naturally mesh with the deep Kuiper Belt
% program described in \autoref{sec:ss:KBO}, although the KBO program
% requires returning to a given field with a much slower cadence than
% that needed to follow supernova light curves. 



==> supernovae/sn-interveningsurveys.tex <==
%\section{Intervening Surveys}
%\label{sec:sn:intervening}
%\noindent{\it Michael Wood-Vasey} % (Writing team)

% ============================================================================
% % - Briefly mention what each of the surveys will contribute
% % - Briefly discuss predictions of near-term results
% % - Decide how this interacts with Nearby Supernovae in the Coming Decade
% % - Should this discussion go before the science topics are introduced?
% %      (i.e. where it currently is?).
% % - Define abbreviations for surveys
% ============================================================================

%There are a number of current and near-future large-scale surveys that
%will start to address the scientific topics here.
%These surveys include 
%KAIT, CSP, CfA, ESSENCE, SNLS, Pan-STARRS1, SkyMapper, DES.
%In particular the nearby searches (KAIT) and follow-up efforts through the Carnegie (CSP) and CfA supernova project will reveal new properties and
%things to investigate in \sneia.  These new discoveries will pose
%new questions that will most likely only add to the list of great supernovae
%questions that will be addressed by the LSST.

%Key Questions that this Chapter should address.
%\begin{enumerate}
%\item What do hundreds of thousands of well-observed \sneia out to $z \sim 1$ get you that ESSENCE, SNLS, Pan-STARRS, SkyMapper, DES, and other efforts won't
%have done? 
%\item How do we do the best job with the systematic errors? 
%\item How do we find the perfect subset of these \sneia for cosmology: e.g.,
%elliptical-only, only galaxies with multiple \sneia (we should
%calculate this number), \sneia in a narrow apparent restframe color
%range found in non-cluster E3 galaxies, etc. 
%\item One key part of this will be a systematic study of the effect of dust on the photometric redshift assigned to SNe.  How does the LSST fit into that?
%\item Comparing spectroscopic and photometric redshifts for a select group of SN would allow an understanding of the systematics for the vast majority of SN that will be measured only
%photometrically. 
%\end{enumerate}



==> supernovae/sn-lowz.tex <==
%\section{Low Redshift Supernovae and Progenitors}
%\label{sec:sn:lowz}
% ============================================================================
% % - The natural complement to having high and moderate-redshift sections
% %    but it's not clear that we're going to keep these
% % - LSST saturates at SN Ia max @ z~1 but lots to do with fainter SNE
% % - SN progenitors.  See, for example, the Pan-STARRS key project on massive stars
% ============================================================================



==> supernovae/sn-nearbysurveys.tex <==
%\section{Nearby Supernovae in the Coming Decade}
%\noindent{\it Robert Kirshner} % (Writing team)
% ============================================================================
% % - Needs discussion of nearby SN surveys 
% % - Plus estimate of state of SN knowledge in 5 years
% ============================================================================



==> supernovae/sn-other.tex <==
% \section{Other SN Types}
% \label{sec:sn:nonsniacosmology}
% 
% Are there possibilities to do distance measurements with other types of supernovae, or possibly even novae?
% 
% \begin{enumerate}
% \item Type Ib/c
%     \begin{enumerate}
%         \item Can we standardize them based on some of their light curve properties?
%     \end{enumerate}
%     \item EPM-equivalent distance to novae in the Milky Way or very nearby galaxies?
% \end{enumerate}
% 


==> supernovae/sn-othersurveys.tex <==
\section{Synergism of LSST SNR Studies with JWST and SOFIA}
% ============================================================================
% % LAUER to edit
% ============================================================================
\label{sec:sn:snr_lsst_others}
\noindent{\it Jeonghee Rho} % (Writing team)

The nucleosynthetic yields and dust formation from supernovae are important and fundamental
astrophysics problems to be solved in the next decade.  Recent deep sub-mm
observations have also shown galaxies and quasars with very large dust
masses ($>10^8 \rm{M_{\odot}}$) at $z>5$ \citep{wang08,beelen06,bertoldi03}.
The time scales for stars to release their dust are too long to explain these
high redshift systems \citep{morgan03}.  In contrast, supernovae produce
copious amounts of heavy elements and release them on short time scales.
Theoretical modeling of the conditions in the supernova ejecta indicate that
Type-II SNe are sources of dust formation and should produce substantial
quantities of dust, on the order of a solar mass per explosion
\citep{dunne03,todini01,nozawa03}.  Yet until very recently, there existed little
observational evidence that this actually occurs. The {\em quantity} of dust
formed within SNe ejecta has become a subject of debate in recent years 
\citep[e.g.,][and references therein]{rho08, dunne09}.  \citet{lagage96}
first showed evidence, in Infrared Space Observatory (ISO) images,
for dust formation in the nearby, young supernova remnant (SNR) Cas A.
\citet{rho08} identified three distinct ejecta dust populations based on their
continuum shapes in Spitzer Space Telescope spectra, including broad
features peaking at  21 $\mu$m  and estimated a total dust mass of between 0.02
to $\rm  0.054\,\rm M_\odot$.  These observations provide definitive evidence
of freshly-formed dust in a young supernova remnant and show that SNe are
important dust contributors to the large quantities of dust observed at high
redshifts.



==> supernovae/sn-physics.tex <==
%\section{The Physics of Supernovae} REMOVED PER SIDNEY WOLFF, 5/19/09
%\noindent{\it Phil Pinto, Patrick Young, Michael Wood-Vasey} % (Writing team)

% ============================================================================
% % - Needs contributions from Pinto and Young
% ============================================================================

%Supernova light-curves will be followed for many years as the supernova ejecta
%expand to reveal the inner workings of the explosions, leading to new
%understanding of the \snia mechanism through, e.g., the interaction with
%the circumstellar environment. Very late-time light-curves can also provide
%additional constraints on host-galaxy reddening using the color constancy
%of their pure iron recombination spectra.

%Core-collapse supernovae provide the instantaneous star formation
%rate, and the LSST will accurately map this rate by finding many tens of
%thousands of these events in the redshift range where it is known that
%the cosmic star formation rate has changed most dramatically.
%Accurate star formation rates will be calibrated as a 
%function of galaxy type and (given spectroscopic follow-up) emission line
%flux.

%The LSST data will enable an accurate determination of the luminosity
%unction of \sneia, which will help constrain progenitor
%models and explain the observed dependence of the luminosity
%distribution of these supernovae with galaxy morphology.

%Core-collapse supernovae are now believed to be the source of
%gamma-ray bursts, but the mechanism producing the bursts remains a
%mystery. Some models predict a delay between the supernovae explosion and
%the formation of the gamma-ray burst, and afterglows provide a variety of
%information on the gamma-ray emission mechanism itself. Testing these ideas
%requires monitoring large areas of the sky to see if a supernova has
%exploded days, weeks, or months earlier (\autoref{chp:transients}). The LSST enables
%natural tests for such models, especially if the delay time scales are
%longer than a few days.

%Some of the physics of supernovae topics that LSST will contribute to:

%\begin{itemize}
%\item Light curve behavior
%\item Luminosity
%\item Color
% \item Features
%\item Diversity of environment
%\item Shock breakout,
%\item Distribution of explosion energies
%\item High-mass progenitor supernovae 
%\item Do pair-production supernova exist? 
%\end{itemize}

%The natural follow-up question will be if these properties evolve with cosmic time: e.g., are they dependent on local environment, metallicity, or host galaxy environment?
 


==> supernovae/sn-presnoutbursts.tex <==
% \section{Pre-supernova Outbursts}
% % ============================================================================
% % %  - Needs work
% % %  - Talk to Smartt about PS1 science case
% % %  - What will LSST be able to do more on this.
% % ============================================================================
% 
% 
% Over the 10 years of the survey, we will have monitoring of supernova
% for years prior to the explosion. We may observe a number of supernova
% such as SN 2006jc for which an outburst was observed two years prior
% to to he SN explosion\citep{pastorello07}.
% %(Pastorello et al., 2007, Nature, Vol. 447, No. 7146, pp. 829-832) 
% Are these specific to Type Ib? Do all types
% exhibit similar phenomena? Is this a common property limited by our
% time-coverage-limited observations or is it only something that
% happens for a small fraction of SNe? This should teach us a lot about
% end-stage stellar evolution and pre-supernova evolution of the
% progenitor systems. 
% 
% 


==> supernovae/sn-sneiin.tex <==

% 2009/05/03 - MWV
% This will be a good section.  Need to get Cooke along with Lien and Fields to flesh this out
% Removing for now.
\section{Type IIn SNe}
\noindent{\it Jeff Cooke} % (Writing team)

Briefly, SNe IIn comprise the brightest SN on record and are the
brightest SN in the FUV (redshifted to the optical at $z > 2$).  In
addition, they have have bright emission lines that are detectable for
many years after outburst that confirm the detections - even at z > 2
(Ly-alpha).  SNe IIn comprise ~3\% of the total SN population and
therefore require wide-field coverage.  I would be happy to email a
detailed discussion of SNe IIn and their detection at high-z, if you
would like.  In the meantime, you might want to check out my paper on
this \citep{cooke08}.
%(2008 ApJ, 677, 137).

The design, filters, depth, and sky coverage of the LSST are well-suited
to detect a very large number of $z > 2$ SNe IIn.  The idea is to stack
images from each year to achieve the necessary depth and to create
yearly light curves for color-selected $z > 2$ galaxies.  I estimate
that the LSST will be sensitive to $\sim10^9$ $z > 2$ galaxies and 
$\sim0.5-2$ $z > 2$ $SNe IIn$ square-degree$^-1$ year$^-1$ (or a few x $10^4$ $z > 2$ SNe IIn year$^-1$, total).

Detections of core-collapse $z > 2$ SNe IIn will progress many areas of
research such as measurements of the supernova and star formation
rates out to high redshift, evolution of Type II supernovae, and
galaxy formation and feedback processes.  With such a large number of
detections, it is very likely that a subset of SNe IIn will have
properties that can be calibrated for cosmological use.  This would
provide a probe of dark energy to test the Type Ia results that would
be effective to even greater distances.

%\subsection{The Power of Supernovae}
%
%\begin{itemize}
%
%\item The LSST data set will give detailed measurements of the
%redshift-distance relation to $z=1$ and perhaps beyond, thus providing
%stringent limits on the equation of state of dark energy, $w$, and its
%evolution. The large number of supernovae will allow a data set to be
%divided up into many subsets consisting of events with identical properties.
%Each subclass will provide an independent estimate of $w$, and consistency
%among them will indicate minimization of systematic effects such as supernovae
%evolution.
%
%If accurate spectroscopic redshifts to hosts can be obtained, then an
%innovative approach based upon the derivative of the Hubble diagram can provide
%an estimate of $w$. This method would have sources of systematic error that are
%complementary to the standard distance/redshift relation technique to give yet
%another check on $w$. {\bf This needs further explanation! I have no idea what
%this means!}
%
%\item The precision in measurement of \sneia means that they
%are powerful probes of the dark matter distribution through weak
%lensing. The supernova complement the technique of mapping mass structures
%using lensing shear discussed in section 7. Supernovae probe higher spatial
%frequencies of the matter power spectrum and are better at defining the
%range in redshifts over which lensing effects are important.
%
%\item 
%
%



==> supernovae/sn-snr.tex <==
\section{Supernova Remnants}
\noindent{\it Jeonghee Rho} % (Writing team)
% % ============================================================================
% % % - Updated draft.
% % % - Needs editing go-through.
% % ============================================================================
% 
% Strongly lensed supernova for time-delays, $H_0$, cluster DM properties
% is in conjunction with the strong lensing working group led by Phil
% Marshall. For more details see Strong Gravitational Lensing. 
% 
% 
*Young supernova remnants:
1) Expansion and motion of ejecta knots for young SNRs such as Cas A,
Tycho, etc:  Multi-epoch observations will allow us to observe
expansion of the forward shocks and the motions of ejecta knots. For
example of Cas A, expansion was measured by 6000 \kms and the knots
typically  move with a velocity of 9000-11000 \kms \citep[e.g.,][]{fesen01}.
The expansion velocity and the motion of  ejecta knots are
equivalent to 0.4"/yr and 0.6-0.7"/yr, respectively. Therefore, we will
observed the knots in Cas A are moving  3-4pixels in an year and and
the SNR shell is moving 2 pixels in a year. For the case of Tycho,  the
expansion rate is 0.41" per year \citep{hughes00}.  With multi
observations, we can make a movie of expansion and eject knots for
young supernova remnants over a long baseline.

*Type II SNe
You already have supernova Physics and supernova progenitors. I think
it would be important to set up a network to make  follow-up
observations with optical spectroscopy, near-IR and mid-IR
observations. I have been working on dust formation and nucleosynthesis
in Type II SNe. How much dust and ejecta are generated by  Type II SNe
are great interests, because huge quantities of dust ($10^8$-$10^9$ Msun)
are observed in very high--redshifted galaxies and quasars 
\citep{isaak02}.  The dust observed in high-redshift galaxies suggests that
dust was produced efficiently in the first generation of supernovae
(SNe). The time scales involved for the dust in the cool, dense  stellar
winds of evolved stars  are far too   long to replenish the dust in our
galaxy \citep{morgan03}.
By followup observations, we can
measure mass of ejecta line emission and dust continuum in infrared. In
near-IR, we should be able to CO fundamental and continuum dust as well
as rich ejecta line emission.
 


==> supernovae/sn-stronglens.tex <==
\section{Strong Lensing of Supernovae}
\label{sec:sn:lensing}
\noindent{\it Masamune Oguri} % (Writing team)
% ============================================================================
% % - Incorporate with future lensing sections
% ============================================================================

%The density of supernovae on the sky is such that we will be able to
%detect the magnification bias due to lensing from individual
%clusters.  Given that we will have precise photometric (and in some
%cases spectroscopic) redshifts for these supernovae, and will
%accurately know the intrinsic (unmagnified) brightnesses of these
%objects, we will be able to put detailed constraints on models of the
%cluster mass distribution.  Closer to the cluster core, supernovae
%will be gravitationally split; we estimate that one in a thousand
%high-redshift supernovae will be strongly lensed by a cluster or
%galaxy.  
%Over the life of the survey, we will discover over 100 SN
%Ia's with multiple images and accurately measured
%time delays.
%The number of supernovae surrounding individual
%clusters is sufficient that they will provide their own weak lensing
%signal, magnification at many points in the sky surrounding mass
%concentrations.  This form of weak lensing will take advantage of the fact
%that the distances to the lensed objects will be known to far better
%precision than the background galaxies usually employed. The sample of type
%Ia supernovae built up in standard LSST operations will also allow us to
%measure $w$ as a function of angle across the sky. 
%A variation in $w$ with direction would have serious implications for
%fundamental physics. 

LSST will discover an enormous number of SNe, and it is reasonable
to assume that some of them will be strongly lensed. These lensing
events have a big advantage over strongly lensed quasars because the intrinsic
brightness of the source is well known; the information of the
magnification factor is helpful to break degeneracies between mass
profiles of lensing galaxies and cosmological parameters
\citep{oguri03}. In addition, the high magnification by lensing allows
us to detect SNe at redshifts well beyond the redshift limit of
un-lensed events. The abundance of such anomalously high redshift SNe can
be a useful probe of high-redshift SN rates. 

We expect to discover over 300 lensed SNe over the life of the
survey, about 30\% of which are lensed \sneia. A more comprehensive
discussion about strongly lensed SNe is given in \autoref{chp:sl}.

%thus allowing much stronger constraints on
%the lensing geometry. Well-modeled, strong lenses 
%provide important constraints on the evolution of galaxy and cluster matter
%distributions, as well as $H_0$, itself an important ingredient in measuring
%the cosmic equation of state.
%In addition, supernovae can be used as a generic weak lensing probe,
%complementing the techniques discussed in \autoref{chp:wl}.
%Indeed, weak lensing effects have been observed in supernovae
%\citep{williams04}; the LSST measurement of the galaxy
%distribution will allow such analyses to be done with great
%precision. 
%They
%probe higher spatial frequencies of the matter power spectrum, and are
%better at defining the range of redshifts over which lensing effects
%are important.  



==> supernovae/sn-surveyrequirements.tex <==
\section{Survey Requirements}
\label{sec:sn:requirements}
{\it DRM} % (Writing team)
% ============================================================================
% % - Revisit and check numbers vs. science cases again
% ============================================================================

To employ the LSST as a true supernova factory requires careful thought
to design requirements for the LSST survey(s). A survey with five filters,
returning to the same field every three or four nights as specified in the
``universal cadence'' (\autoref{sec:sn:cadence}), would cover one-quarter
of the sky per 
cycle. As the year progresses, new fields in the East would replace older
fields in the West, eventually covering most of the visible sky.

A deeper survey reaching $V=26$ and $z=25$, however, requires 10--20
minutes of accumulated exposure in each filter, with revisits of five to
seven days; visits in the different filters need not be done on the same
day. This change in the exposure time from the standard cadence results in
a reduction of $N_{FOV}$ by factors of 30--50. It is therefore necessary to
define some fraction of every night which is devoted to this long exposure
cadence. If that fraction were 10\%, such a program would discover and
study 1,500 \sneia per year out to a redshift $z=1.2$ and a
comparable number of core-collapse supernovae, typically to $z=0.6$ but
with significant numbers to $z>1$ (for example, some progenitors of
gamma-ray bursts such as SN~1998bw). BVRIz light-curves (the $Y$ filter would
be even better with a very red-sensitive detector) would be obtained in
parallel with the search and provide a means of discriminating between
supernova types (with spectroscopic followup of some small fraction of
events to determine reliability). The combined data sets will provide
photometric redshifts to host galaxies.  Work remains to be done to
merge this program with the suggested deep KBO program described in
\autoref{sec:ss:KBO}; as pointed out before, the two need somewhat
different filters (the KBO science really only needs observations in
two filters), and different cadences.  

We touch briefly on other requirements. 

\noindent{\it Photometric Calibration:} Absolute photometric calibration to
2\% is adequate for supernova science. The calibration of the zero
points between filters (the absolute spectrum of Vega is not known to 1\%)
is a serious issue bearing on the subject of K corrections. The stability
of the filter response functions over time (or the frequency of the
measurement of the throughput of the system as a function of
wavelength) is also an issue.   

\noindent{\it Sky Coverage:} To reach the goal of well-sampled light
  curves for hundreds of thousands of supernovae requires observations
  of the high-latitude sky several times per month to $R\sim24$,
  similar to what we've seen in other chapters. 

\noindent{\it Seeing:} Good seeing is important for supernova work, to
  go faint, but more importantly, to separate supernovae
  photometrically from their host 
galaxies.  This is especially important at high redshift, where the
experience with HST is that the photometry is {\em far} superior to what is
obtainable from the ground.  Of course, properly sampled images are
important as well.  Accurate PSF photometry on a complicated background
requires an accurate model for the PSF, which requires that the PSF be
relatively stable as a function of position on the focal plane. There are
no strong requirements on astrometric accuracy.  Like the variability
searches, rapid reduction of the data is important to allow any follow-up
work to be done.

\noindent{\it Auxiliary data:} We have made reference here to
  spectroscopic observations of supernovae obtained on other
  facilities.  The full scope of what is needed here remains to be
  quantified; however, many of the core science goals described in
  this chapter can be achieved with just enough spectroscopic data to
  properly calibrate and test supernova photometric redshift
  techniques.  Indeed, the simulations described above assumed that
  redshifts were determined from supernova light curves, not from
  spectroscopy.  

How much of supernova science is likely to be done by the time the LSST comes
on line?  The largest current high-redshift supernova surveys are the
ESSENCE and CFHT Legacy surveys. ESSENCE is designed to obtain 230
supernovae with $0.2<z<0.75$ to measure $w$ to 10\%. Optical observations
are taken with the CTIO 4m and $zJ$ photometry and spectroscopy are
obtained using various 8m class telescopes.  The CFHT Legacy Survey is
expected to detect about 700~\sneia over a five-year period
with a similar program, and also plans to be able to determine $w$ to
10\%.  Pan-STARRS will discover of order $10^4$ supernovae per year
\citep{tonry03}.
As we have seen, the LSST will obtain orders of magnitude more
supernovae, and determine $w$ to much higher precision.  It is already
known, from WMAP and other analyses, that $w$ is within 20\% of $-1$
(the Cosmological Constant value).
Understanding the physical nature of dark energy requires measuring
any deviation of $w$ from $-1$, and its time and directional
dependence, to superb precision. 

%{\bf We need at least a brief mention of the ``competition'', things
%   like the ESSENCE project and other on-going and planned supernova
%   studies.  And what about the 4-telescope Pan-STARRS?  Can we make
%   the case that these science goals will not all be done by the time
%   the LSST comes on line?
%
%   I don't believe these numbers come even close. 700 supernovae will not
%   get one 10\% in w by my calculations, not even when you don't include
%   all of the various uncertainties like reddening, the fraction of SNe
%   you detect that you can't measure to the stated goal, etc.
%
%   The difference here is hoped-for performance vs an honest appraisal.
%   SNAP expects to get 8\% with 2000 SNe out to z=1.7 (Goliath, Amanulllah,
%   Astier, Goobar, and Pain 2001 astro-ph/0104009, no prior on H0 or
%   OmegaMatter). How can these other surveys get 10\% with z<0.8 and 25\%
%   as many objects observed less accurately?
%
%   I would argue that such a table is somewhat misleading, but probably
%   needs to be included.
%}




==> supernovae/tables/sn_cadence_requirements.tex <==
% ======================================================================
%+
% NAME:
%   supernovae/tables/sn_cadence_requirements.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
\begin{table}
\begin{tabular}{ll}
Science & Cadence \\ 
\hline
Type Ia Supernova Cosmology  & 2 days cadence in at least one filter; \\ 
                             & At least two colors every 4 days; \\
                             & Allowed to miss criteria 3 time in 3 months \\
Isotropy and Homogeneity     & ... \\ 
Cosmology with SNe II        & 3 days cadence in at least one filter; \\
                             & At least two colors; \\
                             & Allowed to miss criteria 6 times in 3 months  \\
Other SNe                    & 3 days cadence in at least two filters for at least 4 months \\
                             & with at least 4 observations a 4th filter separated by one week; \\
                             & 1,000 every 2 days in at least one filter for at least 6 months \\
Type IIn SN Detection and Rates & 4 days cadence in at least two filters  \\
SN Evolution                 & Same as ``Type Ia Supernova Cosmology'' \\
SNIa BAO                     & 10 days cadence  \\
SNIa Photo-z                 & 5 days cadence in at least 2 filters \\
SNIa Weak Lensing            & Same as ``Type Ia Supernova Cosmology'' \\
Moderate Redshift Type II SNe & \\
Low Redshift Supernovae      & \\
Medium Redshift Supernovae   & \\
High Redshift Supernovae     & \\
Pre-supernova Outbursts      & 10 day cadence on nearby galaxies and MW in at least one filter; \\
Supernova Rates              & 30 day cadence in at least 3 filters \\
Supernova Physics            & ??? \\
Supernova Remnants           & No cadence requirements \\
Dark Matter Equation of State & \\
Supernovae and Gravitational Lensing & \\
\end{tabular}
\caption[Supernova Cadence Requirements]{Requirements for cadences to support different supernova science with LSST.}
\label{tab:sn:cadence_requirements}
\end{table}


==> weaklens/references.tex <==
% ======================================================================
%+
% NAME:
%   weaklens/reference.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
\newcommand{\prd}{{\it Phys. Rev. D}}
\begin{thebibliography}{}
\vskip-2in

\bibitem[Haiman, Mohr, \& Holder(2001)]{hmh01}
Haiman, Z., Mohr, J. J., \& Holder, G. P. 2001, \apj, 553, 545

\bibitem[Hamana, Takada, \& Yoshida(2004)]{hty04}
Hamana, T., Takada, M., \& Yoshida, N. 2004, \mnras, 350, 893

\bibitem[{{Heymans} {et~al.}(2006)}]{2006MNRAS.371L..60H}
{Heymans} C. et~al. 2006, MNRAS, 371, L60

\bibitem[{{Hoekstra} et~al.}{2004}]{2004ApJ...606...67H}
{Hoekstra} H.,  {Yee} H.~K.~C.,    {Gladders} M.~D.,  2004, ApJ, 606, 67

\bibitem[Jain \& van Waerbeke(2000)]{jv00}
Jain, B., \& van Waerbeke, L. 2000, \apj, 530, L1

\bibitem[Jenkins et al.(2001)]{jen01}
Jenkins, A., et al. 2001, \mnras, 321, 372

\bibitem[Kratochvil, Haiman, Hui, \& May(2008)]{khhm08}
Kratochvil, J., Haiman, Z., Hui, L. \& May, M. 2008, in preparation.

\bibitem[Lima \& Hu(2005)]{lh05}
Lima, M., \& Hu, W. 2005, \prd, 72, 043006

\bibitem[{{Mandelbaum} {et~al.}(2006a)}]{2006MNRAS.368..715M}
{Mandelbaum} R., {Seljak} U., {Kauffmann} G., {Hirata} C.~M., {Brinkmann} J.,
  2006a, MNRAS, 368, 715

\bibitem[{{Mandelbaum} {et~al.}(2006b)}]{2006MNRAS.370.1008M}
  {Mandelbaum} R., {Hirata} C.~M., {Broderick} T., 
	{Seljak} U.,  {Brinkmann} J., 2006b, MNRAS, 370, 1008

\bibitem[{{Milgrom}}{1983}]{1983ApJ...270..365M}
{Milgrom} M.,  1983, ApJ, 270, 365

\bibitem[{{Parker} {et~al.}(2007)}]{2007ApJ...669...21P}
{Parker} L.~C., {Hoekstra} H., {Hudson} M.~J., {van Waerbeke} L.,
{Mellier} Y., 2007, ApJ, 669, 21

\bibitem[Press \& Schechter(1974)]{ps}
Press, W., \& Schechter, P. 1974, \apj, 187, 425

\bibitem[{{Sackett}}{1999}]{1999ASPC..182..393S}
{Sackett} P.~D.,  1999, in ASP Conf. Ser. 182, p. 393.

\bibitem[{{Sanders}}{1986}]{1986MNRAS.223..539S}
  {Sanders} R.~H.,  1986, MNRAS, 223, 539

\bibitem[Spergel et al.(2007)]{sp07}
Spergel, D. N., et al. 2007, \apj~Suppl. Ser. 170, 377

\bibitem[White, van Waerbeke, \& Mackey(2002)]{wvm02}
White, M., van Waerbeke, L., \& Mackey, J. 2002, \apj, 575, 640

\bibitem[Kaiser \& Squires (1993)]{ks}
Kaiser, N., \& Squires, G. 1993, \apj 404 441.

\bibitem[Tyson, Valdes \& Wenk]{tvw_1990}
Tyson, J.A., Valdes, F., \& Wenk, R. 1990, \apj 349L, 1

\bibitem[Fahlman et al. (1994)]{fahlman94}
Fahlman, G., Kaiser, N., Squires, G. \& Woods D. 1994, \apj 437, 56. 

\bibitem[Fischer et al. (2000)]{Fischer00}
Fischer, P. et  al. 2000, AJ 120, 1198.

\bibitem[McKay et al. (2001)]{Mckay01}
Mckay, T.A. et al. 2001, ASPC 237, 425.

\bibitem[Sheldon et al. (2001)]{Sheldon01}
Sheldon, E. et al. 2001, ApJS 554, 881.  

\bibitem[Mackey et al. (2002)]{Mackey02}
Mackey, J., White, M, \& Kamionkowski, M. 2002, MNDRAS, 332, 788.

\bibitem[Heymans et al. (2004)]{heymans04}
Heymans, C., et al. 2004, MNRAS, 347, 895

\bibitem[Kaiser, Squires \& Broadhurst]{ksb}
Kaiser, N., Squires, G., \& Broadhurst, T. 1995, \apj 449, 460.

\bibitem[Tyson \& Fischer (1995)]{tyson_fischer95}
Tyson, J.A., \& Fischer, P. 1995, \apj 446L, 55.

\bibitem[Seitz (1996)]{Seitz96}
Seitz, S. 1996, IAUS 173, 151.

\bibitem[Seitz, Schneider \& Bartelmann (1998)]{seitz_schneider98}
Seitz, S., \& Schneider, P., \& Bartelmann, M. 1998, A\& Aa 337, 325.

\bibitem[Bradac (2005)]{bradac05}
Bradac, M. et al. 2005, A\& A 437, 49.

\bibitem[Khiabanian \& Dell'Antonio (2008)]{khiab08}
Khiabanian, H., \& Dell'Antonio, I., 2008, ApJ 684, 794.

\bibitem[Clowe et al. (2006)]{clowe}
Clowe, D., et al. 2006, \apj 648L, 109.

\bibitem[Broadhurst, Taylor \& Peacock (1995)]{broadhurst95}
Broadhurst, T.J., Taylor, A.N., \& Peacock, J.A. 1995, MNRAS, 273, 157.

\bibitem[Wittman et al. (2003)]{wittman03}
Wittman, D., et al. 2003, \apj 597, 218.

\bibitem[Jain \& Taylor (2003)]{jt03}
Jain, B., \& Taylor, A. 2003, PhRvL, 91, 1302.

\bibitem[Springel, V. et al. (2005)]{Millenium}
Springel, V. et al. 2005, Nature, 425, 629.

\end{thebibliography}




==> weaklens/testinggravity.tex <==
% ======================================================================
%+
% NAME:
%   weaklens/testinggravity.tex
%
% PURPOSE:
%
%
% COMMENTS:
%
%
%
%
%    
% INPUTS:
%
%
%
% OPTIONAL INPUTS:
%
%
% OUTPUTS:
%
%
% DEPENDENCIES:
%
%
%
%
% EXAMPLES:
%
%
%   
% BUGS:
%
%
% AUTHORS:
%
%
%-
% ======================================================================
{\it Morgan May and Sheng Wang}

A wide variety of cosmological observations, including Type Ia
supernovae surveys, cosmic microwave background (CMB) experiments,
galaxy redshift surveys, and weak gravitational lensing surveys, now
support a single model for the overall architecture of the observable
universe and the development of all structures within it.  According to
this ``concordance model'' \citep{sp07}, the geometry of the observable
universe is almost indistinguishable from a flat geometry, as very early
on, the universe conceivably underwent ``inflation'', a phase of
extremely rapid expansion.  The two dominant components of the universe
appear to be non-baryonic dark matter, whose gravity is responsible for
structure formation, and a mysterious form of dark energy, whose
pressure is currently causing the expansion of the universe to
accelerate.  The mean density of baryonic matter is only about 20\% of
the total amount of matter.

The model explains many different features of the observable universe,
but it is not entirely satisfying.  One of the important issues is that
the origin of the dark energy remains unknown.  We are still far from a
working hypothesis or any significant understanding of cosmic
acceleration.  Two common candidates of dark energy in the literature
are vacuum energy (a cosmological constant) and scalar fields
(quintessence).  However, because the implications of dark energy for
fundamental physics are likely to be profound and revolutionary, we need
to be sure that it is absolutely necessary as an explanation of the
astronomical observations \citep{albrecht_etal06}.

Theoretical alternatives exist to explain the cosmic acceleration, such
as ``modified gravity,'' a modification of general relativity on large
scales.  This includes modifications due to the presence of extra
dimensions, scalar-tensor theories and others.  We are driven to
consider this prospect by potentially deep problems with the other
options.  For instance, a cosmological constant, if not zero, would be
expected to be $10^{120}$ times larger than is observed.  This leaves
unresolved one of the great mysteries of particle physics.  The two
families of models, dark energy and modified gravity, are fundamentally
different, and a question of major importance is to distinguish between
the two possibilities using cosmological data.

One such hope is to look for a possible failure of general relativity
through comparison of the effect of dark energy on cosmic expansion with
the effect of dark energy on the growth of cosmological structures.
Recently, \citet{us07} applied the parameter-splitting technique
\citep{zhs05} on the current data sets.  Given a dark energy parameter,
such as the energy density $\Omega_\Lambda$ or equation of state $w$, it
is split into two parameters with one controlling geometrical distances,
and the other controlling the growth of structure.  Observational data
are then fit without requiring the two parameters to be equal.
\autoref{fig:QCDM} shows the main result from \citet{us07}.  It reveals
no evidence of a discrepancy between the two split meta-parameters.  The
difference is consistent with zero at the $2\sigma$ level for the
quintessence(Q)-CDM model.  The existing data sets already pose tight
constraints on $w$ derived from geometry.  However, the constraint is
much weaker for $w$ derived from growth, because currently galaxy data
are limited by the uncertainty of the bias factor and WL data are
restricted by both the width and depth of the survey.  
LSST will open these windows dramatically.

%
\begin{figure}%[htp]
  \begin{center}
  \includegraphics[width=120mm]{weaklens/qcdm_2d}
  \caption{\label{fig:QCDM}Joint constraints on $w({\rm geom})$ and
    $w({\rm grow})$ in a QCDM model.  The contours show the $68\%$
    confidence limits from the marginalized distributions.  The thick
    gray line shows $w({\rm geom})=w({\rm grow})$.  Different contours
   and curves represent constraints from different combinations of the
    current data sets (CMB, SNe, galaxies and WL).  The smallest contour and the
    most narrow curve (black solid line) represent constraints from all
    the data.  No significant difference is found and deviations are
    constrained to
    $w({\rm geom})-w({\rm grow})=0.37^{+0.37+1.09}_{-0.36-0.53}$ ($68\%$
    and $95\%$ C.L.).  The star-shaped symbol corresponds to the
    effective $w({\rm geom})$ and $w({\rm grow})$, which approximately
    match the expansion history and the growth history, respectively, of
    a flat DGP model with our best-fit $\Omega_m$. Adapted from \citet{us07}.}
  \end{center}
\end{figure}
%

The parameter-splitting technique can also check for 
%%%%inconsistency between different data sets, as well as for
{\it internal} inconsistency within any {\it one} data set, such as
shear tomography, that is sensitive to both geometry and growth.
%The constraints will significantly improve by applying WL data from LSST.
In fact, LSST shear tomography {\it alone} will constrain $w({\rm
geom})-w({\rm grow})$ to 0.04, an order of magnitude better than
current constraints from all data sets \citep{zhs05}.

Parameter splitting can be thought of as a crude way to parameterize
the space of these theories.  As such, the constraints can be viewed
as putting restrictions on modified gravity theories, with the caveat
that the precise constraints on any particular theory must be worked
out on a case by case basis.  \autoref{sec:cp:grav}
and \autoref{sec:cp:newphys} offer more detail on exotic cosmologies and
additional ways that LSST can constrain them, most notably by
combining multiple probes including weak lensing.


